Testing for Balance in Social Networks

Friendship and antipathy exist in concert with one another in real social networks. Despite the role they play in social interactions, antagonistic ties are poorly understood and infrequently measured. One important theory of negative ties that has received relatively little empirical evaluation is balance theory, the codification of the adage `the enemy of my enemy is my friend' and similar sayings. Unbalanced triangles are those with an odd number of negative ties, and the theory posits that such triangles are rare. To test for balance, previous works have utilized a permutation test on the edge signs. The flaw in this method, however, is that it assumes that negative and positive edges are interchangeable. In reality, they could not be more different. Here, we propose a novel test of balance that accounts for this discrepancy and show that our test is more accurate at detecting balance. Along the way, we prove asymptotic normality of the test statistic under our null model, which is of independent interest. Our case study is a novel dataset of signed networks we collected from 32 isolated, rural villages in Honduras. Contrary to previous results, we find that there is only marginal evidence for balance in social tie formation in this setting.

==> Production Ready/Chapters/conclusion.tex <==
%!TEX root = ../main.tex

\section{Conclusion and Future Work}

% Research in social network modelling seems to have reached an impasse -- as the list of fundamental properties is exhausted, 
% social network study feels stuck, we just make more complicated models, to close the gap between theory and practice.
% no fundamental results lately, just more complicated models, to close the gap between theory and practice.
% could this list be exhausted? are there no more fundamental results?
% the study of social networks has reached an impasse - we seem to have exhausted all the simple-to-describe but complex-in-its-emergent-behavior.
% as a result, we have resorted to using more complicated models that do nothing to inform our understanding of social networks.

% The study of social networks has reached an impasse between model and data, and we have resorted to building ever more complicated contraptions to emulate the data.
% There has been a paucity of fundamental results in social network modelling in recent years.
% Almost no fundamental results on social networks have been uncovered of late

% From the paucity of fundamental results on social networks in recent years, it would seem that we have exhausted the simple yet foundational properties that govern social network formation.
% Accordingly, the field has resorted to building increasingly complicated contraptions to close the gap between theory and practice, which provide little in the way of furthering our understanding of social networks.
% It is our contention that the current state of the field is due, in part, to the fact that we completely ignore negative ties in our models.
Models of social network structure and function would benefit from not ignoring negative ties. 
Our hope is that, \hl{in much the same way that moving from $\mathbb{R}$ to $\mathbb{C}$ produces new insights and simplifications}, the extension to signed graphs can provide simple mechanisms to hitherto complicated models.
% Our hope/belief is that, by simply expanding the set of ties that we consider, we may find a simple mechanism that governs the behavior of network structure. Balance theory is a contender for such a mechanism, though there is still work required to see how it fits in with the rest of the mechanisms.

Balance theory is potentially one such mechanism.
In this paper, we introduced a new test for balance that, unlike the standard test currently being used, takes into consideration the different behaviors of negative and positive ties.
We showed through theoretical analysis and simulations that our test outperforms the original.
We applied our test to a novel dataset of village social networks in rural Honduras, and found that balance theory holds true in a minority of the villages, though the villages varied in their extent of balance.

% 1. We think the simple extension to signed graphs is under-developed and much can be learnt

% Social networks in the real world are complicated systems. In spite of this, we have been able to discover fundamental processes that govern different facets of their behavior. 

% The formulation of null models in the context of complex structured data like networks is hard, especially when one is modelling real-life data.
% Social networks in the real world are incredibly dynamic and complex, and yet we have been able to discover fundamental processes that govern parts of their behaviour, even while we have been restricting ourselves to just the positive relationships. What other foundational processes have been potentially hidden in plain sight?

% In this paper, we proposed a new null model for Balance, one that removes the balancing effects, while carefully maintaining the semblance of a realistic social network.
% By taking into account the embeddedness of ties for the permutation, we are able to more accurately measure the presence of balance.
% Additionally, we showed asymptotic normality of our statistic by employing a simple technique of \citet{Janson:2007dx}, with the key insight being that our problem is very similar to the dichotomy between $G(n,p)$ and $G(n,m)$ graphs.

% ========================  Future  ========================  % 

There is much more to be done in this nascent field of understanding and modeling signed social networks.
In addition to the task of understanding the causes of the distribution of balancing effects across social networks, we also have the following future directions:
% In particular:
% \todo{dynamic vs static}
\begin{itemize}
  \item 
  The count of unbalanced triangles is by its very nature a global measure of balance. For reasonable sized graphs such as our village dataset, a global measure is appropriate.
  However, once we move towards much larger social networks -- especially those on the order of, say, Facebook's social graph -- the assumption that there is one measure of balance across the entire graph is no longer tenable. This regime requires a completely new framework for measuring and interpreting balance, the first step of which is to define a new local definition of balance.
  % \item The measures of balance that we and others employ are all global measures. As our dataset involves networks of a sufficiently compact size, a global measure would not be that different from a local one. However, especially in the case of large graphs on the order of magnitude like Facebook's social graph, we should expect variability in the levels of Balance across the graph.
  \item The definition of balance as a function of the product of signs extends effortlessly to higher order cycles. 
  Here, we have restricted our attention to triads, as we think the first order is the most important (and most plausible).
  There has been some work considering higher order cycles \citep{Estrada:2014vb,iosifidis2018}, but little justification for doing so.
  Similarly, while balance theory is the most natural means of relating negative and positive ties, perhaps there are other types of relations possible.
  % \item Having studied and verified the existence of balance, how should we incorporate this into models of social networks? We have preliminary results showing that by the simple addition of balance, models of social networks are able to capture many types of behavior, not least the formation of communities.
  % \item The conclusions we are able to draw
  % \todo{large dataset to then be able to compare with other signed datasets, and make claims about the differences between real life signed graphs and online signed graphs (and similarities)}
  \item Stratification is only one way to account for the differences in negative and positive ties when performing a statistical test.
  An alternative method would be to incorporate existing network models of tie formation, such as exponential random graph models.
  We preferred to adopt a nonparametric approach here to minimize the number of model assumptions, but we leave this potential extension to future work.
  \item In this manuscript, we have considered \emph{undirected} signed graphs.
  One could extend our results to directed graphs, but this leads to a combinatorial explosion in the number of different triangle arrangements, and so one loses the simple interpretation of the 4 different states.
  % , which is the way in which balance theory was first proposed.
  % which are the natural first graph type to consider balance theory.
  % , as this is the fundamental graph type pertaining to balance theory.
  % Moving to directed edges leads to a combinatorial explosion of the number of different arrangements of signed triangles, and so one loses the simple and clean interpretation afforded by undirected triangles.
  Another extension is to consider weighted signed edges, not just binary signed edges. There, the question is how best to generalize the notion of balance in this setting -- one possibility is to take the product of the edges as a measure of the balance of that triangle.
\end{itemize}



==> Production Ready/Chapters/honduras.tex <==
%!TEX root = ../main.tex

\section{Case Study: Villages in Rural Honduras}
\label{sec:data}

% ========================  Related Work  ========================  % 

% \todo{Where do we want to put this section?}
% \subsection{Related Datasets}
% It would be disingenuous to say that we have the first ambisocial dataset, as there are a handful of datasets available that contain both positive and negative ties (for some particular notion of valence).
Signed networks were first studied in the context of international relations: \citet{harary1961structural,moore1979structural} studied several international conflicts, from the Middle Eastern Suez Crisis of 1956 to the Indo-Pakistani War of 1971, while \citet{Antal:2006cia} studied the evolution of alliances during World War I.
Similarly, though at a scale considerably smaller than nation-states, \citet{hage1973graph,Hage1984} studied the New Guinea tribe warfare relations.
The nodes in these signed graphs are all collective entities, as opposed to individuals, and the ties themselves are primarily focused on warfare, rather than simple social engagements.
% They looked at 16 tribes in New Guinea -- having a total population of 12,000 -- and the relations of alliance and opposition between them.

The actual sociocentric mapping of negative ties in parallel with positive ties in social networks is uncommon \citep{Everett:2014cb}.
\citet{rawlings2017structural} examined antagonistic ties in 129 people in a sample of 31 urban communes in the USA from the 1970's, and the classic \citet{sampson1969crisis} study of 18 novitiate monks collected information about members of the group who were disliked. Studies have also mapped helpful and adversarial relationships in small groups in classrooms \citep{huitsing2012bullying,mouttapa2004social} or workplaces \citep{xia2009exploring,Labianca:2006hk}. Other work has examined the networks formed by wild mammals \citep{Ilany:2013ig,lea2010heritable}.


% \hl{The issue with country-level interactions is that they are not a good representation of individual social interactions and the resulting graph size is meagre at best. Thus, these networks are underwhelming from both a sociological and statistical point of view.}

A more recent source of signed networks are those derived from online websites: \citet{Kunegis:2009ks} considered the endorsement graph on the web forum Slashdot; \citet{Guha:2004hs} analyzed the trust/distrust network on the online review website Epinions; and \citet{burke2008mopping} looked at the public voting records for Wikipedia admin candidates.
% that may be less generalizable to real world settings.
Online networks have the advantage of scale (the above networks are on the order of $10^5$ nodes), but their artifically constructed notions of valence make them much less generalizable to real world settings.
% Additionally, the online platform imposes a very limited set of interactions that can be performed. 
% These artificially constructed notions of valence 
% , but they are highly artificial
% Online networks like these -- while massive in size -- are highly artificial; the relationships used are a poor mimicry of real social ties, and the online platform imposes a very limited set of interactions that can be performed.

% The dataset that is closest in spirit to what we have are the New Guinea tribe warfare relations, as set out in \citet{hage1973graph,Hage1984}. They looked at 16 tribes in New Guinea -- having a total population of 12,000 -- and the relations of alliance and opposition between them.
% The vertices, while not as large as nations, are still not individuals. The setting, while not as artificial as an online website, still deals with warfare and not simple social engagements.

% To the best of our knowledge, our dataset, which we present below, is the first capturing both positive and negative ties between individuals in a real social network.


\subsection{Rural Social Networks Study}

% \todo{we don't want to be that precise, because otherwise it'll make people question the dataset, which is not the point here, because we take the dataset as for granted...}

In the summer of 2010, the Rural Social Networks Study (RSNS) collected data on the social networks of around 5000 respondents spread across 32 rural villages in the La Union, Lempira region of Honduras \citep{kim2015social}.
The villages are geographically close to one another but there is little between-village communication.
% ; thus the villages' social networks can be treated as separate units of analysis.
The study gave a small survey to about 87 percent of the respondents in each village before playing a set of economic games.
The survey included a small number of demographic controls and concentrated on ``name generators'' to collect data on the social networks of each village.

For the name generators, the RSNS used a photographic census of all residents, coupled with bespoke software (a much revised version of which, known as \texttt{Trellis}, is available online at \url{http://trellis.yale.edu/}).  This software program was created to use photographs for the identification of ``alters'' to increase accuracy and efficiency of collecting social network data in the field. The photos help solve the name similarity problem. For instance, in one village, there were 16 Maria Hernandezs.


% We collected data from 32 small isolated rural villages in highland Honduras, with an average adult population of 35. % (range 12 to 96, SD=16)
% We conducted a photographic census of all adult inhabitants and used bespoke software to fully (sociocentrically) map the social network \cite{perkins2015social}. We used several \emph{name generators} to discern social ties among participants \cite{shakya2014association}. For example, each respondent was asked who their \emph{closest friends} were, as well as who they \emph{do not like} in their village.
% \todo{add link to appendix}

% mentioning directed vs undirected
% Although the connections being collected could be treated as directed, all of the ties, negative and positive, are treated as symmetrical.
% The name-generators used to ascertain the ties all asked for strong affective relationships which are less likely not to be reciprocated. Negative ties are also so sparse as to make reciprocity unlikely; the data supports this conclusion given that with tens of thousands of connections, only one dyad shares a negative and positive tie.

The name generators primarily focused on receiving strong affective relationships of each respondent: kinship, best friends, and matrimony. But the study also asked a question about ``general dislike''. In all, about 10 percent responded with alters to the negative affective name generator.
% The process for measuring antagonistic ties through self-report was the same as it was for positive ties.
% There are various questions that could be used to tap into different parts or levels of antagonism like hatred or annoyance but we decided that general negative affect is most epitomized by \emph{do-not-like} and that this would be more common.
% Hence, each respondent was asked ``Is there anyone in the community that you don't like?'' followed by a request for the name of that alter.
One of the weaknesses of self-reported antagonistic ties is that people display a reticence to speak negatively of other people in their communities to strangers.
We assume that the actual levels of animosity in these communities are higher than we are able to report because of this social desirability.
% All the ties, negative and positive, are also treated as symmetric
Name generators, by their very nature, produce data that is directional. We shall work with the symmetrized undirected version of this dataset\footnote{This dataset is hosted at our Lab's portal (\url{http://humannaturelab.net/}).}.
% \todo{still feels out of place, this paragraph}
% Some estimates place antagonistic relationship frequency at between 1 and 8 percent of total relationships \citep{Labianca:2006hk}, but these estimates depend on varying methods of measuring relationships and social desirability, and other concerns may influence how many negative relationships a respondent might name \citep{white1961management,labianca1998social}. Online networks generally evince higher percentages of negative ties, if they are allowed or observed, ranging from 15 percent in the Epinions network \citep{Leskovec:2010hw} to 40 percent in an online game network \citep{Szell:2010kf}.
% By its very nature, the name generators create directed ties. 
% \todo{directed ties...}

% ========================  Negative  ========================  % 

\subsection{The Behaviour of Negative Ties}

% To the best of our knowledge, this is the first dataset capturing both positive and negative ties between individuals in a social network.
We begin by considering the negative ties as a separate entity, and compare their behavior to positive ties.
\Cref{fig:villages} shows representative village subgraphs of each type.
% Even usually, there is no mistaking the two.
Clearly there is no mistaking the two.
The positive subgraphs are as expected, conforming to our established ideas of social networks.
Meanwhile, the negative subgraphs are extremely sparse, with most ties being isolated, and almost all the components are trees (i.e. no cycles).
There are instances of cycles, but they are exceedingly rare.
In fact, as hinted earlier, the negative subgraphs bear a striking resemblance instead to sparse random graphs, with their locally tree-like structure.
% These graphs are very sparse and locally tree-like, much like sparse random graphs.

% One is immediately struck by their resemblance to sparse random graphs, having locally tree-like structures.
% There are exceptions to this though that make them decidedly different from random graphs (especially in \cref{subfig:n26}).
% They will sometimes join up to form elaborate shapes, though there are few discernable patterns.
% There is something almost alien about these graphs.
% We shall first consider the behaviour of negative ties as distinct from positive ties, before embarking on the question of their interdependence.
% As this is the first dataset capturing both positive and negative ties in an real social network, it will be instructive to consider the negative ties in isolation first.
% It is natural for our analysis to begin with comparisons to the positive tie behaviour.
% The natural point of reference for negative ties is its positive counterpart, and 

\begin{figure}[h]
  \centering
  % \small
  \begin{subfigure}[b]{.49\textwidth}
    \includegraphics[width=.9\textwidth]{Figures/net-n11.pdf}
    \vspace*{-2em}
    \subcaption{Village \# 11: Negative}
    \label{subfig:n11}
  \end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
    \includegraphics[width=.9\textwidth]{Figures/net-p11.pdf}
    \vspace*{-2em}
    \subcaption{Village \# 11: Positive}
    \label{subfig:p11}
  \end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
    \includegraphics[width=.9\textwidth]{Figures/net-n26.pdf}
    \vspace*{-2em}
    \subcaption{Village \# 26: Negative}
    \label{subfig:n26}
  \end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
    \includegraphics[width=.9\textwidth]{Figures/net-p26.pdf}
    \vspace*{-2em}
    \subcaption{Village \# 26: Positive}
    \label{subfig:p26}
  \end{subfigure}
  \caption{
  Representitive examples of negative and positive subgraphs. In \subref{subfig:p11}, there is evidence of clustering into two communities. On the other hand, the negative subgraphs contain many components of very long trees. The largest component in \subref{subfig:n26}, for instance, would never be mistaken for a positive social network.
  % Comparison between negative subgraphs and random graphs: (a) Village \#22's network, showing only negative ties and removing any resulting empty nodes; (b) the result of an \ER game, $G(n,m)$ with $n=100, m=40$.
  }
  \label{fig:villages}
\end{figure}

More concretely, we calculated various graph statistics aggregated over the 32 villages, which we show in the first two rows of \Cref{tbl:summary_statistics}.
% The first two rows of \cref{tbl:summary_statistics} contain several aggregate graph statistics of these two types.
% [Make some comments regarding the table].
We see that negative ties are much less common than positive ties, exhibit very little transitivity, do not form long connected paths, nor do they coagulate into a giant component -- corroborating our observational conclusions.
In other words, they lack the common features found in positive social networks.
% Clearly, negative ties behave markedly different from positive ties, and
% This further validates the intuition/theory that negative ties will behave differently because there is no network effect.

\begin{table}[h]
  \centering
  \footnotesize
  \begin{threeparttable}
  \begin{tabular}{$l^r^r^r^r^r^r}
    \toprule
    Type & \# Edges & Graph Density & Transitivity & Mean Path Length & \# Components \\ 
    \midrule
    % Neg. & 19.7 & 0.002  & 0.01 & 1.87 & 8.44 & 112.56 \\ 
    % Pos. & 331.9 & 0.056 & 0.26 & 3.59 & 1.66 & 2.19 \\ 
    Pos. & 331.9 & 0.056 & 0.26 & 3.59 & 1.66 \\ 
    Neg. & 19.7 & 0.002 & 0.01 & 1.87 & 8.44 \\ 
    \rowstyle{\itshape} Rnd. & - & - & 0.04 & 1.32 & 13.59 \\ 
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[] \emph{Graph Density} is the ratio of edges to the number of possible edges
  \item[] \emph{\# Components} is the number of non-denegerate components, ignoring isolated vertices
  % \item[] \emph{\# Isol. Vert.} is the number of isolated vertices.
  \end{tablenotes}
  \caption{Average values of select graph statistics across the two subgraphs (positive and negative) of the 32 village networks, as well as an \ER graph with the same number of edges and vertices as the negative subgraph.
  % The column \emph{\# Components} is the number of non-denegerate components, ignoring isolated vertices.
  }
  \label{tbl:summary_statistics}
  \end{threeparttable}
\end{table}

% \todo{rewording this section}

% In fact, one does not need to even check the statistics to reach such a conclusion -- simply staring at a subgraph of negative ties (e.g. \Cref{fig:villages}) reveals that negative ties are closer in kin to (sparse) random graphs. Such graphs exhibit very tree-like local structures, with almost no triangles.



To facilitate the more appropriate comparison with sparse random graphs, we generated, for each negative subgraph, an associated \ER graph under the $G(n,m)$ model with the same $n,m$ as the village graph (where $n$ is the number of nodes, and $m$ is the number of negative ties). The same graph statistics were calculated on this random graph sequence (shown in the third row (\emph{Rnd.}) of \Cref{tbl:summary_statistics}).
As expected, these numbers are very similar to that of the negative subgraphs.
Of particular note is that the transitivity in the random graphs is higher than that from the negative subgraph, suggesting that negative ties might be repelled from forming triangles.


% Another from random graphs is in their in-degree distribution -- the maximum in-degree value across all the villages was 9, compared to only 3 for the random graphs.
% If we were to model negative ties alone, we would probably wish to use a random graph model with a very small probability of being an attractor, but with no network effect.

% The most striking aspect of negative ties, when compared to positive ones, is their close resemblance to random graphs \todo{show negative counterpart, alongside ER graph}. In part because of their relative sparsity, they also lack many of the common features found in positive social networks, such as triadic closure, reciprocity and clustering. This is to be entirely expected, as unlike positive ties, there is no network effect.
% Out of a total of 667 directed negative edges, only 16 pairs where reciprocated.

% \begin{figure}[h]
%   \small
%   \begin{minipage}{.5\textwidth}
%     \centering
%     \hspace*{-3em}
%     \includegraphics[width=1.3\linewidth]{Figures/net-u12.pdf}
%     % \vspace*{-1em}
%     (a) Village (\#12) with all the ties.
%   \end{minipage}%
%   \begin{minipage}{.5\textwidth}
%     \centering
%     \hspace*{-3em}
%     \includegraphics[width=1.3\linewidth]{Figures/net-n12.pdf}
%     (b) Village (\#12) showing only the negative ties.
%   \end{minipage}
%   \caption{Social Network}
%   \label{fig:both}
% \end{figure}

% They are not entirely random though, as indicated by the tail of the degree distribution (cf. \Cref{fig:sep_degree}). In particular, we see that several individuals have large in-degree. This can be explained by the distribution of node characteristics that affect the existence of negative ties, such as general likeability.

% \todo{this section is weird because we use in-degree. I think we should just stick to undirected (?) - because otherwise we have to explain. though we probably should explain such things (!)}



% \begin{figure}[h]
%   \centering
%   \includegraphics[width=1\linewidth]{Figures/dall.pdf}
%   \caption{Degree Distributions}
%   \label{fig:sep_degree}
% \end{figure}

% If we compare the degree distributions between those who received a negative tie to those who gave negative ties [], we see that they have a generally higher degree count than the baseline. In other words, those who were participating in negative relationships -- either actively or passively -- generally had more ties.

% ========================  Dependence  ========================  % 


\subsection{Interdependence between Negative and Positive Ties}

So far, we have considered negative ties in isolation, as an entity separate and independent of their positive counterparts.
However, such independent analysis can only provide a partial picture, as it ignores the positive landscape in which the negative ties are embedded. The same can be said for positive ties.
It is therefore crucial that we understand the interactions between positive and negative ties, as to start building the foundations for a simultaneous model of positive and negative relationships on a network.

% While there is certainly some scholarship to such independent analysis, it can only provide a partial, and quite possibly inaccurate picture, as it ignores the positive landscape in which the negative ties are embedded in. The same can be said for positive ties, though to a lesser extent.
% While there is something to be garnered from such independent studies, it can only provide a partial picture, as it ignores the positive landscape in which it is embedded in. The same can be said for positive ties.

% We tested for structural differences by calculating the average embeddedness of negative ties in the positive graph, and then comparing that to if the signs were permuted. If the placement of negative ties were the same as that of positive ties, there would be no significantly different result after permutation.
% We could have also simply compared it to the average for positive ties (as in []), but then we wouldn't have had a significance value.

% Before we investigate balance, we shall first test for structural differences between negative and postive ties.
Before we investigate balance, let us first test for structural differences between positive and negative ties in the networks. To that end, we shall test for a difference in the average embeddedness levels between the two ties, under the original null model, which we will refer to as the \emph{structural test}. 
We find that 17 graphs are significant at the 5\% level, out of a possible 28 graphs (4 graphs have no negative ties).
This reinforces our claim that negative and positive ties are structurally different.
% Now, when we use the old test for balance, we find that 19 villages are significant at the 5\% level.
More importantly, all 17 graphs found significant in structural differences were also significant for the old test.
If we look at a contingency table between these two tests (\Cref{subtbl:structvstan}), it is clear from the concentration of mass on the diagonal that the old test is essentially a test for structural differences, in disguise.
Thus, if we simply used the old test on this data, the conclusion, erroneously drawn, would be that balance is highly significant.
% Thus, if one were to use the old test, one would 

% \todo{this section needs work (1/2 h)}
% Firstly, we will compare the two types of ties and conclude that they behave differently.
% Then, we will perform three statistical tests per village.
% These are tests for structural differences, the original test, and the new test.
% As we proclaimed earlier, the original test, by not taking into account the different behavior of positive and negative ties, reduces to a test for that difference. This is clearly demonstrated in \Cref{tbl:summary_statistics}.

% \begin{table}[h]
%   \small
%   \centering
%   \begin{tabular}{lrr}
%     \toprule
%     & uniform & stratified \\
%     \midrule
%     5 \% & 19 & 10 \\
%     1 \% & 17 & 7 \\
%     0.5 \% & 13 & 4 \\
%     \bottomrule
%   \end{tabular}
%   \caption{Number of villages falling into a certain significance level.}
%   \label{tbl:counts_sig}
% \end{table}

\begin{table}[h]
  \small
  \centering
  \begin{subtable}{.49\linewidth}
    \centering
    \begin{tabular}{r|cccc}
      % \toprule
      \diagbox{Struct.}{Old} & Not Significant & Significant \\
      \midrule
      Not Significant & 9 & 2 \\
      Significant & 0 & 17 \\
      % \bottomrule
    \end{tabular}
    \caption{Structural vs. Old Test}
    \label{subtbl:structvstan}
  \end{subtable}
  \begin{subtable}{.49\linewidth}
    \centering
    \begin{tabular}{r|cccc}
      % \toprule
      \diagbox{New}{Old} & Not Significant & Significant \\
      \midrule
      Not Significant & 9 & 9 \\
      Significant & 0 & 10 \\
      % \bottomrule
    \end{tabular}
    \caption{New Test vs. Old Test}
    \label{subtbl:stratvsstan}
  \end{subtable}
  % \begin{subtable}{.24\linewidth}
  %   \centering
  %   \begin{tabular}{r|cccc}
  %     % \toprule
  %     1\% & N.S & S \\
  %     \midrule
  %     N.S & 11 & 5 \\
  %     S & 0 & 12 \\
  %     % \bottomrule
  %   \end{tabular}
  %   \caption{Struct. vs. Unif.}
  %   \label{subtbl:structvstan1}
  % \end{subtable}
  % \begin{subtable}{.24\linewidth}
  %   \centering
  %   \begin{tabular}{r|cccc}
  %     % \toprule
  %     1\% & N.S. & S \\
  %     \midrule
  %     N.S. & 11 & 9 \\
  %     S. & 0 & 8 \\
  %     % \bottomrule
  %   \end{tabular}
  %   \caption{Strat. vs. Unif.}
  %   \label{subtbl:stratvsstan1}
  % \end{subtable}
  \caption{Contigency table between the various tests.}
  % \textbf{N.S.} Not Significant; \textbf{S.} Significant, where significance is defined at the 5 \% level.}
  \label{tbl:cont_table_sig}
\end{table}

% Applying our new test to the dataset, we see that balance is in fact, not so ubiquitous.
% In contrast, half as many villages are found to be significant (5\%) under the new test.
Applying our new test to the dataset, we find that at the 5\% level, instead of the 19 graphs found significant from the old test, only half of them are actually significant.
The exact significance levels are shown in \Cref{tbl:individual_sig}.
While there is sufficient evidence to reject the null hypothesis that these social networks do not follow balance, it is clear that balance is not a ubiquitous force. In fact, with only a minority of villages exhibiting balance, the natural question then arises of what makes some social networks more receptive to balancing forces than others.
% This we leave to future work.
% \todo{talk about what conclusions happened in the previous works}
% If we take the significance as a proxy for the level of balance in a village, we see that balance varies quite a bit across the villages, though
% We make no strong claims of a sociological nature.

\begin{table}
  \centering
  \begin{threeparttable}
  \small
  \begin{tabular}{$l^l^l^l^l^l^l}
    \toprule
    ID & \multicolumn{2}{l}{Old} & \multicolumn{2}{l}{Structural} & \multicolumn{2}{l}{New} \\ 
    \midrule
  1 & 0.15 & \scriptsize{ } & 0.14 & \scriptsize{ } & 1.00 & \scriptsize{ } \\ 
    2 & 0.22 & \scriptsize{ } & 0.37 & \scriptsize{ } & 0.31 & \scriptsize{ } \\ 
    4 & 0.19 & \scriptsize{ } & 0.19 & \scriptsize{ } & 1.00 & \scriptsize{ } \\ 
    5 & 0.00 & \scriptsize{$\ast\ast$} & 0.02 & \scriptsize{$\ast$} & 0.01 & \scriptsize{$\ast$} \\ 
    \rowstyle{\bfseries} 6 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.07 & \scriptsize{.} \\ 
    7 & 0.24 & \scriptsize{ } & 0.22 & \scriptsize{ } & 1.00 & \scriptsize{ } \\ 
    \rowstyle{\bfseries} 8 & 0.01 & \scriptsize{$\ast$} & 0.01 & \scriptsize{$\ast$} & 1.00 & \scriptsize{ } \\ 
    9 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.06 & \scriptsize{.} & 0.00 & \scriptsize{$\ast{\ast}\ast$} \\ 
    10 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.01 & \scriptsize{$\ast\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} \\ 
    \rowstyle{\bfseries} 11 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.36 & \scriptsize{ } \\ 
    12 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.01 & \scriptsize{$\ast\ast$} & 0.02 & \scriptsize{$\ast$} \\ 
    13 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast\ast$} \\ 
    14 & 0.10 & \scriptsize{ } & 0.25 & \scriptsize{ } & 0.14 & \scriptsize{ } \\ 
    15 & 0.24 & \scriptsize{ } & 0.50 & \scriptsize{ } & 0.22 & \scriptsize{ } \\ 
    \rowstyle{\bfseries} 16 & 0.04 & \scriptsize{$\ast$} & 0.04 & \scriptsize{$\ast$} & 1.00 & \scriptsize{ } \\ 
    19 & 0.07 & \scriptsize{.} & 0.38 & \scriptsize{ } & 0.06 & \scriptsize{.} \\ 
    20 & 0.52 & \scriptsize{ } & 0.51 & \scriptsize{ } & 1.00 & \scriptsize{ } \\ 
    21 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.03 & \scriptsize{$\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} \\ 
    \rowstyle{\bfseries} 22 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.39 & \scriptsize{ } \\ 
    23 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.01 & \scriptsize{$\ast$} \\ 
    \rowstyle{\bfseries} 24 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.06 & \scriptsize{.} \\ 
    \rowstyle{\bfseries} 25 & 0.01 & \scriptsize{$\ast\ast$} & 0.01 & \scriptsize{$\ast\ast$} & 1.00 & \scriptsize{ } \\ 
    26 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.00 & \scriptsize{$\ast\ast$} \\ 
    \rowstyle{\bfseries} 27 & 0.00 & \scriptsize{$\ast\ast$} & 0.00 & \scriptsize{$\ast\ast$} & 1.00 & \scriptsize{ } \\ 
    28 & 0.29 & \scriptsize{ } & 0.27 & \scriptsize{ } & 1.00 & \scriptsize{ } \\ 
    29 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.06 & \scriptsize{.} & 0.00 & \scriptsize{$\ast\ast$} \\ 
    30 & 0.00 & \scriptsize{$\ast{\ast}\ast$} & 0.01 & \scriptsize{$\ast\ast$} & 0.00 & \scriptsize{$\ast{\ast}\ast$} \\ 
    \rowstyle{\bfseries} 31 & 0.01 & \scriptsize{$\ast\ast$} & 0.04 & \scriptsize{$\ast$} & 0.07 & \scriptsize{.} \\ 
     \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[] .~---~$0.05 \leq p < 0.1$, *~---~$0.01 \leq p < 0.05$, **~---~$0.005 \leq p < 0.01$,
  \item[] ***~---~$0 \leq p < 0.005$
  \end{tablenotes}
  \caption{%
  Table showing the results of three statistical tests on each village network.
  The nine rows in bold are those where the old test is significant while the new one is not.}
  \label{tbl:individual_sig}
  \end{threeparttable}
\end{table}

% conclusion?

==> Production Ready/Chapters/introduction.tex <==
%!TEX root = ../main.tex

\section{Introduction}

Models of social network structure generally build on assumptions about myopic agents, whereby global network features emerge from the dynamic local decision rules of individual agents \citep{holland1998emergence,Kossinets:2006je}. For instance, if agents tend to attach to more central or popular actors, scaling emerges in the degree distribution of the graph \citep{Barabasi:1999je};
if people generally form connections with those who are similar, social networks exhibit homophily \citep{mcpherson2001birds};
if agents form infrequent but random connections with other agents, the social graph has a small diameter, following the small-world phenomenon \citep{Watts:1998db}.

All of these models, however, are restrictive in that they only apply to positive ties.
Much less is theorized or known about the fundamental properties of negative ties.
In principle, they need not share the same structural properties as their positive counterparts.
Moreover, as most social graphs are \emph{signed} (i.e. have both positive and negative ties), this raises the question of how the presence of the negative ties affects the surrounding positive network structure, and how we should model them concurrently.

% ========================  Balance  ========================  % 

\topic{defining balance}
One important theory of negative ties advanced by \citet{Heider:1946vz} relates to an agent's desire for balance in social relationships \citep{Harary:1959ct,simmel2010conflict}. Balance theory postulates that a need for cognitive consistency leads agents to seek to balance the valence in their local social systems.
Simply stated, friends should have the same friends and the same enemies.
This translates, in graph-theoretic terms, to requiring the product of the signs on a triangle to be positive.
Triangles that violate this property are deemed \emph{unbalanced}, and the theory posits that such triangles should be rare compared to their \emph{balanced} counterparts.

\topic{is balance real?}
Balance theory is very simple to state and almost self-evident in nature.
After all, it has already been assimilated into the wider culture through such aphorisms as \emph{``the enemy of my enemy is my friend''}.
However, as evidenced by the success of behavioral economics \citep{kahneman1979prospect}, human actors
will often act irrationally, even so far as to violate transitivity \citep{tversky1981framing}. It is therefore not unreasonable to envisage people violating transitivity in their social graph.

\topic{little evidence for balance}
As it stands, balance theory has received sparing empirical evaluation.
Tests of balance theory require the observation of antagonistic connections between actors, but these ties are often either ignored when the data is gathered, or simply unavailable due to the unwillingness of the actors themselves to divulge such information.
Those studies which have been able to observe antagonistic ties have often done so in artificial settings -- and have been very liberal about what constitutes an antagonistic tie -- like nominations to adminship on Wikipedia \citep{Leskovec:2010hw}, and user ratings of trustworthiness in an e-commerce website \citep{Guha:2004hs}, rather than in face-to-face settings, with some exceptions \citep{mouttapa2004social,huitsing2012bullying,xia2009exploring}.

\topic{test for balance, why sucks}
Though the underlying datasets may be vastly different, these studies all resort to exactly the same statistical test to verify balance in their signed networks:
for the test statistic, they use the number of balanced triangles as a measure of the degree of balance in a graph;
the null model corresponds to a permutation test on the edge weights of the observed graph.
Drawing samples from the null distribution then reduces to shuffling the signs on the graph.
The simplicity of this null model belies its principal flaw though -- namely, that it treats negative and positive ties as interchangeable.
The problem is that, as we shall soon demonstrate, negative ties behave remarkably like random ties drawn from an \ER graph.
% Meanwhile, we already know from decades of research on social networks that positive ties behave nothing like \ER graphs.
On the other hand, researchers have spent the past few decades documenting the various ways that a network of positive ties differs from an Erd\H{o}s-R\'{e}nyi graph.
% Meanwhile, the area of social network modelling was inspired, in part, by the fact that real social networks are fundamentally different to those generated from the Erd\H{o}s-R\'{e}nyi graph model, and so we strive to document the ways in which such disparaties (positive) social networks differ from such random graphs.
% Erd\H{o}s-R\'{e}nyi graphs.

Features like preferential attachment and clustering are fundamental to our understanding of positive ties -- features that are clearly absent in negative ties.
Thus, by treating positive and negative ties as exchangeable, this null hypothesis creates a test, not for balance, but for differences in the behavior of positive and negative ties.

\topic{data example}
As an example, consider one of the social networks from our Honduras dataset, shown in \Cref{fig:intro_network}.
Decomposing the graph into its signed subgraphs reveals \subref{subfig:p22} a typical positive social network, and \subref{subfig:n22} a negative subgraph that could be easily mistaken for a sample from a random graph model.
The contrast between the two subgraphs could not be more extreme, and clearly indicates that these two types of ties should not be treated as exchangeable.

\begin{figure}[h]
  \small
  \begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=1.2\textwidth]{Figures/net-u22.pdf}
    \vspace*{2em}
    \subcaption{Signed Graph}
    \label{subfig:u22}
  \end{subfigure}
  \begin{subfigure}[b]{.5\textwidth}
    \centering
    \includegraphics[width=.9\textwidth]{Figures/net-p22.pdf}
    \vspace*{-2em}
    \subcaption{Positive Subgraph}
    \label{subfig:p22}
    \centering
    \includegraphics[width=.8\textwidth]{Figures/net-n22.pdf}
    \vspace*{-1em}
    \subcaption{Negative Subgraph}
    \label{subfig:n22}
  \end{subfigure}
  \caption{\subref{subfig:u22} A signed social network (Village \# 22).
  Much has been studied about the positive subgraph \subref{subfig:p22}, but very little is known about the negative subgraph \subref{subfig:n22}. The example here suggests that the negative subgraph behaves more like a random graph.}
  \label{fig:intro_network}
\end{figure}

\topic{careful of null hypothesis}
As the ``replication crisis'' \citep{open2015estimating} plays out in the scientific community, and notions like p-hacking and ``garden of forking paths'' \citep{gelman2013garden} become mainstream, one overlooked but equally important issue
is the selection of an appropriate null hypothesis.
In most settings, there is a canonical choice for the null hypothesis.
On the other hand, in the context of complex social data such as social networks, we no longer have this luxury,
as it is difficult to accurately model such data with a simple parametric model.
In this regime, it is imperative to choose null models carefully.

% ========================  Our Contribution  ========================  % 

\topic{our contribution: new null model}
The main contribution of this paper is to provide a new null model that resolves the issues raised above.
The crux of the solution is the following key observation: a crucial way in which negative and positive ties differ is through their \emph{embeddedness} level (the number of triangles that tie is a member of) --
transitivity and homophily encourage higher levels of embeddedness in positive ties.
For instance, the average embeddedness of positive ties and negative ties in the network shown in \Cref{fig:intro_network} was $1.2$ and $0.5$, respectively.
Our new method, therefore, is to stratify the permutation across embeddedness levels, thereby ensuring that the embeddedness profiles of negative and positive ties remain invariant. This preserves the fundamental differences between the two kinds of ties, creating a more accurate null model of a signed social network without balance.
This is supported by both our simulation studies and our theoretical results, where we show that for a reasonable definition of absence of balance in a graph,
the true type-I error rate of the old test converges to 1 while the type-I error rate for the new test is consistent with the specified $\alpha$.

% ========================  Theory  ========================  % 

\topic{describe theory}
To compare the relative performance of the two tests, we show asymptotic normality of the test statistic under the two null models.
Due to the stratified nature of the permutation, this is a nontrivial result, and, to the best of our knowledge, this is the first result showing asymptotic normality of this type of graph statistic under a stratified permutation model.
The key insight is that a distribution derived from a permutation test -- even a stratified permutation -- can be obtained as conditional distribution of independent random variables.
This is similar to the dichotomy between the $G(n,p)$ and $G(n,m)$ random graph model \citep{janson2011random}.
Under certain conditions, the limit and the conditioning operation may be interchanged, enabling us to carry the central limit theorem result in the independent case to the permutation case.
This proof technique of \citet{Janson:2007dx} has wide applicability, not least in the nascent field of (nonparametric) inference on random graphs.

Our final contribution is that we analyze a comprehensive dataset capturing both positive and negative ties between individuals in a social network -- namely, the networks of 32 villages in rural Honduras \citep{kim2015social}.
This novel dataset provides a first look into the behavior of interaction between negative and positive human relationships.
We find that negative ties behave very differently from positive ties.
Applying our new test of balance to the village networks reveals that balance barely registers as an underlying mechanism dictating the structure of signed networks, which is contrary to the conclusions drawn from the previous literature.

\subsection{Organization}

The rest of the paper is organized as follows.
In \Cref{sec:method}, we formally introduce the notion of balance, describe the old null model, its fundamental flaws, and our proposed new null model.
We prove asymptotic normality of the test statistic under both null models in \Cref{sec:theory}, and from this, we show that the new test has a lower type-I error rate than the old test.
This is also supported by the simulation studies we perform in \Cref{sec:simulations}.
Finally, in \Cref{sec:data}, we analyze the networks of 32 rural villages in Honduras.

==> Production Ready/Chapters/method.tex <==
%!TEX root = ../main.tex

\section{Method}
\label{sec:method}

% \subsection{Notation}

% ========================  Balance  ========================  % 
% \subsection{Method}

\topic{defining balance and the consequences}
The theory of balance is an old theory, predating many of the ``classic'' celebrated ideas in social network analysis.
First proposed in \citet{Heider:1946vz}, it was later made formal by \citet{Cartwright:1956dh},
who recast the theory into the more natural graph-theoretic framework.
Adopting such a framework, let us first fix some notation.
% Formally,
Assume that we are given an undirected signed graph $G = (V,E,W)$, where
\begin{itemize}
  \item $V,E$ are vertex and edge sets, respectively, with sizes given by $|V| = N$, $|E| = n$;
  \item $W \in \left\{ -1, +1 \right\}^{n}$ is a vector of edge signs.
\end{itemize}
Let $\triangle, \triangle'$ be the ordered and unordered triplet of indices that form a triangle in $G$, respectively:
\begin{align}
  \triangle &\coloneqq \left\{ (i,j,k) \in E^{3}: i,j,k \text{ form a triangle} \right\}, \\
  \triangle' &\coloneqq  \left\{ (i,j,k) \in E^{3}: i,j,k \text{ form a triangle};\, i < j < k \right\}.
\end{align}
Then, the number of triangles in $G$ is equal to $\abs{\triangle'}$, while $\abs{\triangle} = 6 \abs{\triangle'}$.
For a triangle $(i,j,k)$ in $\triangle$, we say it is \textit{balanced} if $W_i W_j W_k = 1$, and unbalanced otherwise.
% Given a signed undirected graph $G$, they define a triangle to be \emph{unbalanced} if the product of the signs of the edges is negative ($-1$).
Specifically, the unbalanced triangles are those with one or three negative ties ($t_1$ and $t_3$ in \Cref{fig:baltriangles}, respectively), while the remaining two are balanced.
The graph $G$ is then deemed \textit{balanced} if all the realized triangles of $G$ are balanced -- that is,
\begin{align}
  G \text{ is balanced} \iff W_i W_j W_k = 1, \quad \forall (i,j,k) \in \triangle
\end{align}
A simple consequence of this definition is that $G$ is balanced if and only if it can be decomposed into two positive subgraphs that are joined by only negative edges (see \citet{Cartwright:1956dh}).
Finally, a key property of edges that will play a central role in our analysis is its embeddedness, which we define below.
\begin{defn}
  The \emph{embeddedness} of an edge $i \in E$, which we denote by $\varepsilon_{i}$, is the number of triangles that edge $i$ is a part of:
  \begin{align}
    \varepsilon_{i} \coloneqq \frac{1}{2} \sum_{(j,k) \in E^2} \I{ (i,j,k) \in \triangle}.
  \end{align}
\end{defn}

\begin{figure}[h]
  \small
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/t0.pdf}\\
    % (A)
  \end{minipage}%
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/t1.pdf}\\
    % (B)
  \end{minipage}
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/t2.pdf}\\
    % (C)
  \end{minipage}%
  \begin{minipage}{.25\textwidth}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/t3.pdf}\\
    % (D)
  \end{minipage}
  \caption{The four possible arrangements of positive and negative ties in a triangle with undirected ties. Balance theory states that $t_1$ and $t_3$, with an uneven number of negative ties, are unbalanced.}
  \label{fig:baltriangles}
\end{figure}

\topic{psychological background for balance}
One theorized psychological mechanism for balance theory is \emph{cognitive dissonance}, the state of mental strain a person experiences while holding two conflicting beliefs.
This theory holds that it requires high cognitive load to feel both animosity and goodwill towards others \citep{festinger1962theory}.
For instance, in the case of $t_1$ (\Cref{fig:baltriangles}), $Y$ holds negative feelings towards $Z$, but also, by transitivity through $X$, $Y$ should possess positive feelings towards $Z$, leading to cognitive dissonance.
Balance theory posits that, to avoid the cognitive strain from imbalance, individuals ($Y$) will take measures to resolve such inconsistencies in their local social system,
such as switching the valence of their own relationships (befriend $Z$ instead).
On the other hand, agents may choose to simply ignore the facts that are in conflict.
The literature on \emph{cognitive biases} --
e.g. the work of \citet{tversky1981framing} who showed that people are capable of violating the transitivity of their own preferences
-- suggests that individuals might be unperturbed by, or simply unaware of, such inconsistencies or lack the willpower to correct their local systems.

Here, we adopt the frequentist approach favored by the existing literature and devise a hypothesis test for balance theory.
Two ingredients are needed to specify such a test:
a test statistic that measures the balance on a graph, and a null model that describes a graph without balance.
We begin with the choice of a measure of balance.
It is immediately obvious that the binary definition of balance from \citet{Cartwright:1956dh} is highly impractical, as almost every social graph is equally ``not balanced'' under this definition, even though some graphs are clearly more balanced than others.
A more appropriate measure, and the one used throughout this literature, is the number of unbalanced triangles, as higher levels of balance should result in fewer unbalanced triangles.\footnote{The ratio of unbalanced triangles to all triangles would seem like a more appropriate statistic, but since we are ultimately performing a statistical test with a null model that leaves the number of triangles invariant, using the ratio is therefore equivalent to using just the numerator.}
This count, however, is meaningless on its own.

The second and more important choice is the null model that describes a graph without balance, and it is here that we diverge from the current literature. 
Despite the broad spectrum of application settings, the existing literature is unanimous in its choice of a null model.
This null model corresponds to one derived from a \emph{permutation test}, where the permutation is over the signs of the edges on the graph.
To generate a graph under this null model, we simply shuffle the signs on the observed graph.
An equivalent formulation is the following generative model. Start with a positive social graph ($G$), and suppose that negative ties are only ever formed by switching the signs of positive ties. With a fixed budget of $m$ negative ties, generate a graph by picking $m$ ties at random to switch.

To see why this describes a graph without balance, note that balance is a statement about the relation between negative and positive ties, and makes claims about their relative positions on the graph.
Thus, a generative model where the sign of an edge is independent of its position on the graph is necessarily absent of balance.

Having chosen a null model (and a test statistic), the test for balance is now fully specified. For an input graph $G$, we test for balance by comparing the number of unbalanced triangles in $G$ against the distribution of the same statistic under the null model.
The details of the general testing procedure are shown in \Cref{alg:balance}, and the details for this test can be found in \Cref{alg:perm_old}.
Note that this is a \emph{left-tailed} test, as the presence of balance should reduce the number of unbalanced triangles.

Formally, the test statistic that we use to measure balance is the number of unbalanced triangles, given by
\begin{align}
  U \coloneqq \sum_{(i,j,k) \in \triangle'} \I{W_{i} W_{j} W_{k} = -1}.
\end{align}
Denote by $\tau$ a random variable which is uniformly distributed over the set of all permutations of $E$ -- namely over the symmetric group $S_n$ (of size $n!$). This enables us to define a random weight vector $W_{\tau}$ by $(W_{\tau})_i = W_{\tau(i)}$.
Then, the old null model is equivalent to the graph-valued random variable given by $G_{\tau} = (V, E, W_{\tau})$
\footnote{This uniform random permutation is technically \hl{overkill}, as it actually only has an effective size of $\binom{n}{m}$, where $m$ is the number of negative ties, since we are only permutating the signs around.}.
We shall use $G_{\tau}$ interchangeably to mean either the random variable or the associated probability distribution over signed graphs.

\begin{modl}[Old Model]\label{modl:old}
  The graph has distribution $G_{\tau}$, where $\tau$ is uniformly distributed over $S_{n}$.
\end{modl}
The old null hypothesis then corresponds to $H_{0}^{\tau}\colon \mathbf{G} \sim G_{\tau}$, while the number of unbalanced triangles now takes the form
\begin{align}
  U_{\tau} \coloneqq \sum_{(i,j,k) \in \triangle'} \I{ W_{\tau(i)} W_{\tau(j)} W_{\tau(k)} = -1 }.
\end{align}


\begin{algorithm}
\small
\caption{General Test for Balance}\label{alg:balance}
\begin{algorithmic}[1]
\Procedure{TestBalance}{$G$, $N$, \textsc{NullModel}} \Comment{$N$ is the number of simulations}
  \State $r \gets$ \Call{TestStatistic}{$G$} \Comment{observed statistic}
  \For{$i\gets 1$ to $N$}
    \State $\hat{G} \gets$ \Call{NullModel}{$G$} \Comment{generate a graph under the null model}
    \State $s[i] \gets $ \Call{TestStatistic}{$\hat{G}$} \Comment{calculate the statistic on the new graph}
  \EndFor
  \State \Return the fraction of $s \leq r$ \Comment{calculate the $p$-value}
\EndProcedure
\Statex
\Function{TestStatistic}{$G$} \Comment{unbalanced triangle count}
  \State \Return the number of triangles in $G$ that have an odd number of negative ties
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\small
\caption{The Old Test}\label{alg:perm_old}
\begin{algorithmic}[1]
\Procedure{OldTest}{$G$, $N$}
  \State \Return \Call{TestBalance}{$G$, $N$, \Call{UniformPermute}{$G$}}
\EndProcedure
\Statex
\Procedure{UniformPermute}{$G$}
  \State \Return \Call{PermuteSign}{$G, \operatorname{edges}(G)$}
\EndProcedure
\Statex
\Function{PermuteSign}{$G, E$} \Comment{$E$ is a subset of the edges of $G$}
  \State Permute the signs on the edge set $E$ of $G$ at random
  \State \Return $G$
\EndFunction
\end{algorithmic}
\end{algorithm}

This choice of null model has several flaws, however.
First, it confines the formation of negative ties to switches from the existing positive edges, and so prohibits the formation of negative ties from locations where there are currently no edges.
However, this type of behavior might have \hl{some semblance to reality},
as it can be said that having negative feelings towards someone presupposes that you know them well enough to dislike them. Additionally, if we do not restrict the negative edges to the support, we then need to make a judgement as to how the presence of edges should be modeled, which introduces even more subjectivity to the null model.

A more concerning issue is that this null model treats negative and positive ties as interchangeable.
This raises two problems.
The first is that such an assumption is strictly stronger than assuming there is no balance.
Indeed, the two types of ties being exchangeable is equivalent to the sign of an edge being independent of its location, which necessarily implies that there is no balance.
Hence, this null model is in fact testing a stronger statement than lack of balance, leading to a potentially inflated type-I error.
\todo{try to incorporate the idea of conservative test, extent of conservatism}

The second problem is that such an assumption is unrealistic.
On the one hand, researchers have spent the past few decades cataloging the various ways in which positive social networks differ from \ER graphs.
Social networks from a wide variety of settings have been found to share structural similarities \citep{Apicella:2012dt}, such as degree assortativity, transitivity, and homophily -- all properties patently absent in \ER graphs.
On the other hand, as we demonstrate in \Cref{sec:data}, the negative tie subgraph behaves remarkably similar to a random graph.
Thus, by assuming that negative and positive ties are exchangeable, the existing literature has chosen a test that is essentially condemned to significance.

% ========================  Algorithm  ========================  % 

Our main methodological contribution is that we devise a new null model that addresses the aforementioned problems:
% , through an appropriate adjustment to the permutation procedure.
instead of having a uniform permutation across all edges, we stratify the permutation across edges of the same embeddedness.
% That is, for each embeddedness level, we independently perform a uniform permutation across the subset of edges having that level of embeddedness.
Formally, the new null hypothesis differs from the old null hypothesis in the choice of random permutation.
Instead of the random permutation $\tau$, which is uniformly distributed over all permutations of $E$, the new random variable, which we denote by $\pi$, is a (disjoint) composition of uniform permutations, one for each level of embeddedness.
\begin{modl}[New Model]\label{modl:new}
  The graph has distribution $G_{\pi}$, where $\pi$ is given by
\begin{align}
  \pi (E) \coloneqq \left( \tau_{L} \circ \ldots \circ \tau_{1} \right) (E),
\end{align}
where $L$ is the maximum embeddedness level of $G$, and $\tau_{l}$ is uniformly distributed over permutations of the set of edges with embeddedness $l$, denoted by $E_l$, and all other edges are untouched.
\end{modl}
\begin{rmk}
  Note that we do not include the permutation $\tau_0$ (targeting edges which are not part of any triangle) in $\pi$, since such a permutation would not change the graph (and in particular, would not change the number of unbalanced triangles).
\end{rmk}
The new null hypothesis is now $H_0^{\pi}\colon \mathbf{G} \sim G_{\pi}$,
and the corresponding test statistic is given by
\begin{align}
  U_{\pi} = \sum_{(i,j,k) \in \triangle'} \I{ W_{\tau_{\varepsilon_i}(i)} W_{\tau_{\varepsilon_j}(j)} W_{\tau_{\varepsilon_k}(k)} = -1 }.
\end{align}
Define $n_l$ to be the number of edges of embeddedness $l$ and $m_l$ to be the number of negative edges of embeddedness $l$:
\begin{align}
  n_l &= \sum_{i \in E} \I{\varepsilon_i = l}, \\
  m_l &= \sum_{i \in E} \I{\varepsilon_i = l, W_i = -1}.
\end{align}
Note that $\pi$ is determined completely by $\left\{ n_l \right\}_{l = 0}^{L}$.

The exact steps of this procedure are described by the function \textsc{StratifiedPermute} in \Cref{alg:perm_new}.
Crucially, this stratified permutation leaves the embeddedness profile of both negative and positive ties invariant.
As a result, we maintain the embeddedness profiles of both types of tie, while still ensuring there is enough flexibility to garner meaningful variability as a model of a signed network without balance.
Essentially, we argue that ties are only exchangeable at the same embeddedness level.

\begin{algorithm}
\small
\caption{The New Test}\label{alg:perm_new}
\begin{algorithmic}[1]
\Procedure{NewTest}{$G$, $N$}
  \State \Return \Call{TestBalance}{$G$, $N$, \Call{StratifiedPermute}{$G$}}
\EndProcedure
\Statex
\Procedure{StratifiedPermute}{$G$}
  \State $tc \gets$ the triangle membership count for each edge \Comment{e.g. $tc = (1, 1, 3, 3, 0, 4)$}
  \State $utc \gets$ $\operatorname{unique}(tc)$, the unique counts in $tc$ \Comment{e.g. $utc = (1,3,0,4)$}
  \For{$t$ in $utc$}
    \State $E \gets$ the edges in $G$ with triangle count $t$
    \State $G \gets$ \Call{PermuteSign}{$G, E$}
  \EndFor
  \State \Return $G$
\EndProcedure
\Statex
\Function{PermuteSign}{$G, E$} \Comment{$E$ is a subset of the edges of $G$}
  \State Permute the signs on the edge set $E$ of $G$ at random
  \State \Return $G$
\EndFunction
\end{algorithmic}
\end{algorithm}

\vskip1em
The computational cost of the two procedures can be broken down into two tasks: the enumeration of all the triangles in the graph, and the determination of the null distribution of the statistic.
The first part is essentially unchanged by the new stratified test.
In particular, it turns out there is a very straightforward way of calculating both the embeddedness level of edge $(i,j)$ and unbalanced triangle counts: letting $A$ be the signed adjacency matrix corresponding to $G$, we have
\begin{align}
  \mathcal{E}_{ij}&=\left(\left|A\right|\circ\left|A\right|^{2}\right)_{ij}, \\
  U_{n}&=\frac{1}{12}\text{tr}\left(\left|A\right|^{3}-A^{3}\right)=\frac{1}{12}\text{tr}\left(\mathcal{E}\one\one'-A^{3}\right),
\end{align}
where $\one \in \mathbb{R}^{N}$ is a vector of all ones.
It is clear, however, that our method will be more computationally intensive compared to the original test for the latter part, as now we must perform (at most) $L$ permutations for each draw from the null distribution.
For large enough graphs, where Monte Carlo simulations are prohibitively expensive, these considerations are modulated by the fact that our limit theorem demonstrates that a normal approximation of the null distribution suffices.

\topic{shortcomings}
A potential shortcoming of our method is that, since it operates at the embeddedness level, networks where many of the embeddedness levels have only one sign edge type will not have an expressive null distribution.
A simple adjustment is the following: instead of permuting edges across embeddedness levels, we can permute across ranges of levels, which allows signs to hop to different levels.
The question then arises of how to construct the bins.

\topic{Example showcasing the difference between the two tests}
To clearly delineate the differences between our new model and the old model, consider a toy example shown in \Cref{fig:toy2}.
In this social network, there is a core group of six individuals that have formed a clique, as well as an additional three individuals on the periphery that have formed unbalanced triangles with the core group.
We claim that this network is not balanced, and so a statistical test should not reject the null that there is no balance. One might argue on the contrary, as there are more balanced triangles than unbalanced ones. However, the clique should not be treated as evidence for balance, as it can already be explained by transitivity.
\todo{come up with a better example? it's hard}
For instance, a graph with no negative ties is ``balanced'' in that there are no unbalanced triangles, but this is clearly not strong evidence supporting the full spectrum of balance. That is why the key triangles to monitor are those with negative ties ($t_1, t_2, t_3$ in \Cref{fig:baltriangles}).

Applying the old test (\cref{subfig:toy2-1}), which ignores embeddedness levels, we see that it allows the negative ties free rein over the entire support of the graph, including to the dense cluster in the middle, where the embeddedness level is 5. This results in an artificially inflated mean of the null distribution.
On the other hand, our test (\cref{subfig:toy2-2}) restricts this edge to those positions with also embeddedness level of 1, shown in blue.
The old test incorrectly rejects the null, while the new test does not.

\begin{figure}[h]
  \small
  \begin{subfigure}[b]{.49\textwidth}
    \hspace*{2em}
    \includegraphics[width=.75\textwidth]{Figures/toy2-2.pdf}
    \vspace*{-1em}
    \subcaption{Old (Uniform)}
    \label{subfig:toy2-1}
  \end{subfigure}
  \begin{subfigure}[b]{.49\textwidth}
    \hspace*{2em}
    \includegraphics[width=.75\textwidth]{Figures/toy2-1.pdf}
    \vspace*{-1em}
    \subcaption{New (Stratified)}
    \label{subfig:toy2-2}
  \end{subfigure}
  \caption{Comparison of the two permutations. The blue edges correspond to the positions where the negative (red) edges are able to be moved to under the different tests.}
  \label{fig:toy2}
\end{figure}

\topic{discussion of dynamic vs static}
Finally, we discuss the apparent dynamic nature of balance.
The intuitive interpretation of balance presents itself as a dynamic process, one where individuals notice an unbalanced state and then correct it.
An appropriate test of balance would then involve monitoring the evolution of a graph to see if such local corrections are observed. Ignoring the difficulty of obtaining dynamic graph data, we claim that this dynamic analysis is problematic, as balance is not necessarily expressed in discrete steps.
Consider the first scenario in \Cref{fig:dynamic}, which shows a graph entering and leaving an unbalanced state. If we were to capture all three states, we would flag this as an example of balance at play.
Suppose, however, that the window of time between events 1 and 2 is smaller than the resolution of the graph evolution samples. We would then recover scenario two of \Cref{fig:dynamic} instead, which would not be flagged as evidence for balance under a dynamic model, even though there was a local correction.
Thus, as tempting as it may be to treat balance in terms of dynamic local corrections, we think it is more appropriate to consider balance as a holistic property of a graph.
\hl{Of course, the relative timing of data collection compared to the underlying social process is crucial here.}

\begin{figure}[h]
  \centering
  \includegraphics[width=0.7\linewidth]{Figures/scenarios.pdf}
  \caption{Dynamics of Balance. Two scenarios that start and end in the same balanced state, but the intermediary steps are different.
  }
  \label{fig:dynamic}
\end{figure}

% % ========================  Formal Treatment  ========================  % 

% \subsection{Graph-theoretic Formulation}

% Formally,
% assume that we are given an undirected signed graph $G = (V,E,W)$, where
% \begin{itemize}
%   \item $V,E$ are vertex and edge sets, respectively, with sizes given by $|V| = N$, $|E| = n$;
%   \item $W \in \left\{ -1, +1 \right\}^{n}$ is a vector of edge signs.
% \end{itemize}
% Let $\triangle, \triangle'$ be the ordered and unordered triplet of indices that form a triangle in $G$, respectively:
% \begin{align}
%   \triangle &\coloneqq \left\{ (i,j,k) \in E^{3}: i,j,k \text{ form a triangle} \right\}, \\
%   \triangle' &\coloneqq  \left\{ (i,j,k) \in E^{3}: i,j,k \text{ form a triangle};\, i < j < k \right\}.
% \end{align}
% Then, the number of triangles in $G$ is equal to $\abs{\triangle'}$, while $\abs{\triangle} = 6 \abs{\triangle'}$.
% The test statistic that we use to measure balance is the number of unbalanced triangles, given by
% \begin{align}
%   U \coloneqq \sum_{(i,j,k) \in \triangle'} \I{W_{i} W_{j} W_{k} = -1}.
% \end{align}
% One key property of edges that will play a central role in our analysis is its embeddedness, which we define below.
% \begin{defn}
%   The \emph{embeddedness} of an edge $i \in E$, which we denote by $\varepsilon_{i}$, is the number of triangles that edge $i$ is a part of:
%   \begin{align}
%     \varepsilon_{i} \coloneqq \frac{1}{2} \sum_{(j,k) \in E^2} \I{ (i,j,k) \in \triangle}.
%   \end{align}
% \end{defn}

% Denote by $\tau$ a random variable which is uniformly distributed over the set of all permutations of $E$ -- namely over the symmetric group $S_n$ (of size $n!$). This enables us to define a random weight vector $W_{\tau}$ by $(W_{\tau})_i = W_{\tau(i)}$.
% Then, the old null model is equivalent to the graph-valued random variable given by $G_{\tau} = (V, E, W_{\tau})$
% \footnote{This uniform random permutation is technically \hl{overkill}, as it actually only has an effective size of $\binom{n}{m}$, where $m$ is the number of negative ties, since we are only permutating the signs around.}.
% We shall use $G_{\tau}$ interchangeably to mean either the random variable or the associated probability distribution over signed graphs.

% \begin{modl}[Old Model]\label{modl:old}
%   The graph has distribution $G_{\tau}$, where $\tau$ is uniformly distributed over $S_{n}$.
% \end{modl}
% The old null hypothesis then corresponds to $H_{0}^{\tau}\colon \mathbf{G} \sim G_{\tau}$, while the number of unbalanced triangles now takes the form
% \begin{align}
%   U_{\tau} \coloneqq \sum_{(i,j,k) \in \triangle'} \I{ W_{\tau(i)} W_{\tau(j)} W_{\tau(k)} = -1 }.
% \end{align}
% The new null hypothesis differs from the old null hypothesis in the choice of random permutation.
% Instead of being uniformly distributed over all permutations of $E$, the new random variable, which we denote by $\pi$, is a (disjoint) composition of uniform permutations, one for each level of embeddedness.
% \begin{modl}[New Model]\label{modl:new}
%   The graph has distribution $G_{\pi}$, where $\pi$ is given by
% \begin{align}
%   \pi (E) \coloneqq \left( \tau_{L} \circ \ldots \circ \tau_{1} \right) (E),
% \end{align}
% where $L$ is the maximum embeddedness level of $G$, and $\tau_{l}$ is uniformly distributed over permutations of the set of edges with embeddedness $l$, denoted by $E_l$, and all other edges are untouched.
% \end{modl}
% The new null hypothesis is now $H_0^{\pi}\colon \mathbf{G} \sim G_{\pi}$,
% and the corresponding test statistic is given by
% \begin{align}
%   U_{\pi} = \sum_{(i,j,k) \in \triangle'} \I{ W_{\tau_{\varepsilon_i}(i)} W_{\tau_{\varepsilon_j}(j)} W_{\tau_{\varepsilon_k}(k)} = -1 }.
% \end{align}
% Note that $\pi$ is determined completely by the set $\left\{ (m_l, n_l) \right\}_{l = 0}^{L}$, where $n_l$ is the number of edges of embeddedness $l$ and $m_l$ is the number of negative edges of embeddedness $l$:
% \begin{align}
%   n_l &= \sum_{i \in E} \I{\varepsilon_i = l}, \\
%   m_l &= \sum_{i \in E} \I{\varepsilon_i = l, W_i = -1}.
% \end{align}

==> Production Ready/Chapters/simulation.tex <==
%!TEX root = ../main.tex

\section{Simulations}
\label{sec:simulations}

In this section, we first provide empirical verification of our theoretical results showing asymptotic normality of the statistic under \Cref{modl:new}, the stratified permutation null model.
% The rest of the section is dedicated to comparing the performance of the two tests in simulation studies.
The rest of the section is then dedicated to comparing the performance of the tests under generative models of graphs without balance $(H_0)$ as well as graphs with balance $(H_1)$.
Under models of balance-free graphs,
we show that our test is non-significant, while the old test exhibits spurious significance.
% In the case where there is no balance, we show that our test remains non-significant, while the old test can exhibit spurious significance.
This corroborates with our analysis of the Type-I error in \Cref{sub:comparing_both}.
Finally, we simulate graphs with balance, and show that our test maintains the same level of statistical power as the old test. Since our test is generally more conservative, this is the best result possible.

% As our test is a generally more conservative test than the old one, we do not expect to outperform the old test on \hl{both fronts}.
% But at least we show that this new test is not just a uniformly more conservative test.
% The \hl{other side of the coin} is measuring the power of the test -- we demonstrate that our test is not losing power even while it is decreasing Type-I error.

% well that was wrong...
% It is clear from the construction of our null model that our test is a (strictly) more conservative test than the original test.
% Thus, there are only two regimes that we need to consider: (1) if there is no balance ($H_0$), our method should not be significant, while the original test can exhibit spurious significance (increased specificity); (2) if there is balance in the graphs ($H_1$), our method should also be significant (no loss of statistical power).
% We will show that our test is not simply a uniformly more conservative test, but in fact dominates the original test.


\subsection{Asymptotic Distribution}
% we basically had three different distributions
We generated three progressively larger graphs from a Watts-Strogatz model \citep{Watts:1998db}, with parameters given in \Cref{tbl:exact_sw}, and then randomly assigned a fraction of these edges to be negative.
The Watts--Strogatz model, with parameters ($d, n, k, p$), has the following generative mechanism. Form a $d$-dimensional lattice with $n$ nodes per dimension. Then, connect two vertices together if the number of hops on the original lattice between them is at most $k$.
Finally, iterating over each edge, rewire each end with probability $p$.
We ran $10^4$ Monte Carlo simulations to calculate the empirical distribution of the number of unbalanced triangles under $H^{\pi}_{0}$.
% We ran $10^4$ Monte Carlo simulations of the distribution under \Cref{modl:new} on progressively larger base graphs drawn
% from 
% Watts-Strogatz model \citep{Watts:1998db}, with the parameters given in \Cref{tbl:exact_sw}.
These empirical distributions are shown in \Cref{fig:exact}, where we see a clear trend towards convergence to normality.
\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth]{Figures/exact-smallworld.pdf}
  \caption{Histogram of the sample null distribution given the three base graphs, with the density curve of a standard Normal distribution superimposed.}
  \label{fig:exact}
\end{figure}
\begin{table}[h]
  \small
  \centering
  \begin{tabular}{lrrrrr}
    \toprule
    & \emph{d} & \emph{n} & \emph{k} & $p$ \\
    \midrule
    $n \approx 10^3$ & 3 & 4 & 3 & 0.2 \\
    $n \approx 10^4$ & 3 & 6 & 3 & 0.2 \\
    $n \approx 10^5$ & 5 & 10 & 5 & 0.1 \\
    \bottomrule
  \end{tabular}
  \caption{Parameters used in each model of the Watts-Strogatz graph.}
  \label{tbl:exact_sw}
\end{table}

\subsection{Performance Comparisons}

\subsubsection{Comparison under \texorpdfstring{$H_0$}{H0}}

To ensure a fair comparison, we chose different models of balance-free graphs from the permutation based models our tests use.
% The null hypotheses we have analyzed use permutations to simulate no balance, but that is not the only way to simulate a balance-free graph.
% To simulate a graph with no balance, 
% we opted to differ from the method we employed in our null hypothesis, which is to permute the signs on a graph, to ensure that we are not just overfitting to a specific type of \emph{balance-free} model.
% Our generating process is to superimpose a negative \ER graph onto a positive graph. This results in the two edge sets being independent, and hence produces a graph that is balance-free.
Our generating process is to generate positive and negative subgraphs independently (on the same vertex set), and then combine the graphs together, in such a way that the negative subgraph takes precedence. By this procedure, the positive and negative edge sets will be independent, which by definition produces a balance-free graph.

The negative subgraph will be simply drawn from an \ER model (turning all edges to negative ones).
% A simple alternative is to randomly draw the positive and negative subgraphs independently, and then combine the two graphs%
% \footnote{More precisely, provided the negative subgraph is drawn from an independent graph model, and the negative subgraph takes precedent in the event of edge clashes during the combination step, this produces a balance-free graph.
% }.
% We will use an \ER model as the negative subgraph.
For the positive subgraph model, we would like to use a graph model that is a faithful representation of real-life social networks. Here we present two choices:

\textsc{Choice 1: Small-world}.
In this simulation model, we generate the positive part of the social network from the Watts-Strogatz model \citep{Watts:1998db}.
% instead of taking it directly from the data, and keep the negative subgraph augmentation step the same.

The model parameters we used in this simulation are \emph{d} $=1$, \emph{n} $=100$, \emph{k} $=2$, and we varied the rewiring probabilities from $p=0.1, 0.2, 0.3$.
We draw $10^3$ samples each from three instances of the above generative model, and compare the $p$-values the two tests produce, the histograms of which are shown in \Cref{fig:hist_sw}.
For a rewiring probability of $p = 0.1$, we find that the old test is rejecting all $10^3$ graphs, at a significance value of 0\%. On the other hand, the new test rejects the null only 10\% of the time.
As we increase $p$, the graph becomes more like an \ER graph, and the two tests tend towards uniformity, though from opposite directions. Crucially, in all three instances of $p$, our new test is conservative about rejecting the null, while the old test is not.
\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth]{Figures/hist-sw.pdf}
  \caption{Histogram of the $p$-value for differing parameters of the Watts-Strogatz model}
  \label{fig:hist_sw}
\end{figure}

\textsc{Choice 2: Real Data}.
A simple way to ensure that the positive subgraph possesses the features we see in real data is
to just use real data.
% Instead of modelling a realistic social graph, 
We simply removed the negative edges from the social networks we collected, leaving a positive subgraph.
% Given the difficulty of simulating, via a generative model, a social network that possesses the features we see in the real world, one solution is to use the actual social networks we gathered as a basis for the model.
% To do so, we remove the existing negative ties from the social network to form the positive subgraph.
% we removed the existing negative ties from the graph, leaving a positive subgraph.
The negative \ER graph is then added.
% The negative subgraph is an \ER graph with an edge weight of $-1$ onto the same node set of the social network.
% As discussed, this procedure is balance-free, since a graph where the positive and negative ties are generated independently \hl{necessarily} does not exhibit balance.
Selecting three representative villages, we draw $10^3$ samples each from the three resulting models and compare the $p$-values we get from the two tests. The histograms are shown in \Cref{fig:hist_village}.
We see a similar story across the villages, with the old test rejecting very often, while the new test almost never rejects. \todo{maybe some conclusion here?}

\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth]{Figures/hist-village.pdf}
  \caption{Histogram of the $p$-values for a sample of the village networks (\#2, \#12, \#29).}
  \label{fig:hist_village}
\end{figure}

\subsubsection{Comparison under \texorpdfstring{$H_1$}{H1}}

% Having obtained compelling evidence that our method has higher specificity, we now show that sensitivity of our new test is preserved. In order to do that, we must decide on how best to model a graph that now displays balance.

In order to derive a model of a graph with balance,
it will be informative to revisit the original definition of balance in \citep{Heider:1946vz}. There,
a graph is balanced if and only if it can be decomposed into two ``communities'' such that positives ties are within communities and negative ties are between.
Define a signed stochastic blockmodel as the combination of two stochastic blockmodels (SBM) over the same community structure, one for each sign\footnote{Clashes between two edges are deemed as void.}.
For notational convenience, we shall only consider the symmetric 2-community model. Let the parameters of the two SBMs be given by
\begin{align}
  B^{+} = 
  \begin{bmatrix}
    p^{+} & q^{+} \\
    q^{+} & p^{+}
  \end{bmatrix} &&
  B^{-} =
  \begin{bmatrix}
    p^{-} & q^{-} \\
    q^{-} & p^{-}
  \end{bmatrix} &
\end{align}
Then, balance corresponds to $q^{+} = p^{-} = 0$. On the other hand, the graph is balance-free when $p^{+} = q^{+}$ and $p^{-} = q^{-}$. A natural solution to modeling a graph with balance is therefore one where the parameteres are somewhere between the two degenerate solutions.

% To derive a model of a graph with balance, it will be informative to consider the extreme example provided by the original definition of a balanced graph in \citet{Heider:1946vz}. As we mentioned in \Cref{sec:method}, a consequence of such a definition is that a graph is balanced if and only if it can be decomposed into two ``communities'' such that positive ties are within community and negative ties are between.
% This observation motivates the following generative graph model. Define a signed stochastic blockmodel by

% Motivated by the observation that a fully (weakly) balanced graph reduces to a graph of disjoint communities where the within-group ties are positive and the between-group ties are negative, our approach to this modelling task is to generate two stochastic blockmodels (SBM) over the same community structure, one for each sign, where, crucially, the inequality between within-group and between-group probabilities is reversed in the negative subgraph, so that between-group ties are more probable.

% For notational convenience, we shall only consider the symmetric 2-community model. Let the parameters of the two SBMs be given by
% \begin{align}
%   B^{+} = 
%   \begin{bmatrix}
%     p^{+} & q^{+} \\
%     q^{+} & p^{+}
%   \end{bmatrix} &&
%   B^{-} =
%   \begin{bmatrix}
%     p^{-} & q^{-} \\
%     q^{-} & p^{-}
%   \end{bmatrix} &
% \end{align}
% Then, $p^{+} > q^{+}$ and $q^{-} > p^{-}$, and the procedure for generating the graph is outlined in \Cref{proc:sbm}.

% \todo{do we really need this simple algorithm stated?}
% \begin{algorithm}
%   \small
%   \caption{Generating a graph with balance}
%   \label{proc:sbm}
%   \begin{algorithmic}[1]
%   \Function{SignedSBM}{$B^{+}$, $B^{-}$, $c$} \Comment{$c$ is the community size vector}
%     \State $G^{+} \gets$ \Call{SampleSBM}{$B^{+}$, $c$}
%     \State $G^{-} \gets$ \Call{SampleSBM}{$B^{-}$, $c$}
%     \State $A \gets$ \Call{AdjacencyMatrix}{$G^{+}$} - \Call{AdjacencyMatrix}{$G^{-}$}
%     \State \Return \Call{GraphFromAdjacency}{$A$}
%   \EndFunction
%   \end{algorithmic}
% \end{algorithm}

We ran the model with three different sets of parameters (see \Cref{tbl:sim_sbm_params}), and the histograms of $p$-values are shown in \Cref{fig:hist_sbm}. The distribution of $p$-values in the presence of balance are the same across the two methods, which demonstrates that our method doesn't lose out on statistical power. Compared to Model 1 and 2, the level of balance in Model 3 is much lower, and accordingly, the tests are more uncertain, leading to a more uniform distribution.

\begin{table}[h]
  \small
  \centering
  \begin{tabular}{lrrrrr}
    \toprule
    & $n$ & $p^{+}$ & $q^{+}$ & $p^{-}$ & $q^{-}$ \\
    \midrule
    Model 1 & 100 & 0.4 & 0.1 & 0.03 & 0.1 \\
    Model 2 & 50 & 0.3 & 0 & 0 & 0.3 \\
    Model 3 & 50 & 0.3 & 0.2 & 0.2 & 0.3 \\
    \bottomrule
  \end{tabular}
  \caption{Parameters used in each model of the signed SBM.}
  \label{tbl:sim_sbm_params}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=.8\linewidth]{Figures/hist-sbm.pdf}
  \caption{Histogram of the $p$-values from testing for balance in the signed SBM.}
  \label{fig:hist_sbm}
\end{figure}

==> Production Ready/Chapters/theory.tex <==
%!TEX root = ../main.tex

\section{Asymptotics of the Null Distribution}
\label{sec:theory}

One drawback of a permutation test is that the accompanying null distribution has no closed form. Monte~Carlo methods are required to approximate the distribution, and, for large graphs, the number of samples needed for an accurate approximation might be prohibitive. Additionally, the lack of a closed form makes it difficult to compare different null distributions.
We resolve both issues by showing that our statistic, namely, the number of unbalanced triangles, is asymptotically normal under the new null hypothesis, and therefore can be reasonably approximated by a normal distribution with known moments
\footnote{Ideally, we would have a Berry-Esseen type result here to quantify precisely the error in the normal approximation. We leave this for future work.}.
This is the main theoretical result of the paper (\Cref{thm:main}).
% Mostly importantly, this allows us to approximate the null distribution by its first two moments, thereby enabling us to 
% One of the drawbacks of a permutation based statistic is that it requires the use of Monte~Carlo draws in order to approximate the null distribution, and for large graphs, we might expect needing a very large sample in order to have an accurate representation of the null distribution.
% If, however, we could show asymptotic normality of our statistic, and have closed forms for the first two moments, we would be able to sidestep the problem of Monte~Carlo simulations, and instead simply use the normal approximation. That, indeed, is what we show in this section.

% The main theoretical result is the following:


% Given the nature of the null hypothesis, one must resort to Monte Carlo simulations in order to determine the null distribution, and subsequently, the significance level.
% The asymptotic result suggests that calculating the mean and variance suffices.

% The main disadvantage to working with permutation based statistics is that we are no longer dealing with a sum of independent random variables.
The distribution of sums of permutation-based random variables are notoriously difficult to analyze as the random variables themselves are no longer independent.
Thankfully, there is already a whole field dedicated to these types of results, known as combinatorial central limit theorems.
This field was founded by Hoeffding in his seminal paper \citep{Hoeffding:1951im}, in which he utilized the method of moments. Subsequent results have used variations of Stein's method to prove more general combinatorial CLTs (see \citet{Barbour:1989bt}).
While it is a relatively straightforward exercise to extend the results of \citet{Barbour:2005vl} to show asymptotic normality under the old null hypothesis, the additional structure introduced by our stratified permutation renders this approach infeasible.
% our new null model introduces complications to the model
% the problem is that our stratified permutation introduces further complications to the model by having multiple concurrent permutations.

Inspired by the results of \citet{Janson:2007dx}, we instead take a completely different approach.
The key insight is that the distribution of the stratified permutation model is a conditional distribution of a much simpler model, where the signs are distributed as independent (non-symmetric) Rademacher random variables, and the conditioning is on the number of negative ties in each stratum.
% This is akin to the dichotomy between the $G(n,p)$ and $G(n,m)$ graph models.

% Put another way, if we introduce randomness into the problem, in this case randomizing the number of negative ties in each stratum (akin to Poissonization, but in this case we have finite sample size, so Binomization is the more appropriate term), we can potentially bystep the dependent structure of the permutations.
\subsection{Notation}
Fix a signed graph $G = (V, E, W)$. 
%Recall that $G_{\pi}$, which we defined in \Cref{modl:new}, is the null distribution under stratified permutation, and is parameterized by $\left\{ m_l, n_l \right\}_{l = 0}^{L}$.
We can associate with $G$ a new graph-valued random variable, $G_{p} = (V, E, X)$, having the same support as $G$, but with a random weight vector $X$ comprising of independent (non-symmetric) Rademacher random variables. Concretely, the weight vector $X$ is given by $X_i \sim \operatorname{Rad}\left( 1 - p_{\varepsilon_i} \right)$, with $\P{ X_i = 1 } = 1 - p_{\varepsilon_i}, \P{ X_i = -1 } = p_{\varepsilon_i}$, where $p_{\varepsilon_i} = \frac{m_{\varepsilon_i}}{n_{\varepsilon_i}}$.
By construction, edges of the same embeddedness level will have the same probability of being negative under $G_{p}$. The statistic for $G_p$ corresponds to
%\begin{align}
%  V^{(n)}_{p}
%  \coloneqq \frac{1}{2}\left( \abs{\triangle'} - \sum_{(i,j,k) \in \triangle'} X_i X_j X_k \right).
%\end{align}
\begin{align}
  V_{p} \coloneqq \sum_{(i,j,k) \in \triangle'} \I{X_{i} X_{j} X_{k} = -1}.
\end{align}
% in order to have a similar form as for the U's. Then mention in the proof that we can also write it in a different way, which is better suited for calculations.
% and we have the following relationship between $U^{(n)}_{\pi}$ and $V^{(n)}_{p}$:
% \todo{introduce lemma}
\subsection{Main Results}

The relation between $G_p$ and $G_\pi$ is given by the following Lemma.
\begin{lem}\label{lem:cond_dist}
  Denote by $M_l$ the number of negative ties with embeddedness $l$ in $G_p$. Then the distribution of $G_{\pi}$ is just the conditional distribution of $G_{p}$, conditional on the event $M=\bm{m}$, where $M=\left\{ M_l \right\}_{l=0}^{L}$ and  $\bm{m}=\left\{ m_l \right\}_{l=0}^{L}$. In particular,
  \begin{align}
    \mathcal{L}\left( U_{\pi} \right) = \mathcal{L}\left( V_p \,\mid\, M=\bm{m} \right).
  \end{align}
\end{lem}
The proof is deferred to \Cref{sec:appendix_lemmas}.
With respect to proving a CLT we must first define a sequence of graphs. Let $\left\{ G^{(n)} \right\}_{n=1}^{\infty}$ be a fixed sequence of signed graphs, indexed by the number of edges. Then, $G_\pi, G_p$ extend naturally to sequences of graph-valued random variables, $\left\{ G^{(n)}_{\pi} \right\}_{n=1}^{\infty}, \left\{ G^{(n)}_{p} \right\}_{n=1}^{\infty}$ with statistics $\left\{ U_\pi^{(n)} \right\}_{n=1}^{\infty}, \left\{ V_p^{(n)} \right\}_{n=1}^{\infty}$. To simplify notation, we will sometimes drop the index $n$. For instance, we still write $E_l$, $\pi$ and $p_l, m_l$, keeping in mind the dependence on $n$.

\Cref{lem:cond_dist} suggests that we can obtain a CLT for $U^{(n)}_\pi$ by proving one for $V^{(n)}_p$, which should be much easier by independence of edges in $G^{(n)}_p$. In general, however, weak convergence does not imply \emph{conditional} weak convergence. The crucial property that enables one to interchange conditioning and limits is \emph{stochastic monotonicity}, which we define below. Here, we use the partial order $x \leq y$ for vectors $x, y \in \mathbb{R}^{d}$ defined by $x_i \leq y_i$ for all $i$.
% \todo{Change the notation here to match our examples, because otherwise it's too confusing}
\begin{defn}\label{defn:stochastic_monot}
  Let $V \in \mathbb{R}^{q}$ and $M \in \mathbb{R}^{r}$ be random vectors. We say that $V$ is \emph{stochastically increasing} with respect to $M$ if the conditional distribution $\mathcal{L}(V \,\mid\, M = \bm{m})$ is increasing in $\bm{m}$. That is, if for any $v \in \mathbb{R}^{q}$ and $\bm{m}_1 \leq \bm{m}_2$, we have
  \begin{align}
    \P{V \leq v \,\mid\, M = \bm{m}_1} \geq \P{ V \leq v \,\mid\, M = \bm{m}_2}.
  \end{align}
  We say that $V$ is \emph{stochastically decreasing} with respect to $M$ if $-V$ is stochastically increasing with respect to $M$, and $V$ is \emph{stochastically monotone} with respect to $M$ if it is either stochastically increasing or decreasing with respect to $M$.
\end{defn}

Based on stochastic monotonicity it is indeed possible to transform weak convergence to conditional weak convergence. This beautiful result is known as \emph{Nerman's Theorem} (\citet{Nerman:1998fx,Janson:2007dx}).
\begin{thm}[Nerman's Theorem]\label{thm:nermans_theorem}
  Let $V^{(n)} \in \mathbb{R}^{q}$ and $M^{(n)} \in \mathbb{R}^{r}$ be random vectors such that $V^{(n)}$ is stochastically monotone with respect to $M^{(n)}$. Assume that
  \begin{align}
    (a_{n}^{-1} ( V^{(n)} - b_n), c_{n}^{-1}( M^{(n)} - d_n)) \xrightarrow{\mathcal{D}} (V,M)
  \end{align}
  for random vectors $V \in \mathbb{R}^{q}, M \in \mathbb{R}^{r}$ and $a_n, c_n > 0, b_n \in \mathbb{R}^{q}, d_n \in \mathbb{R}^{r}$. Let also $m_n \in \mathbb{R}^{r}$ be a sequence such that $c_n^{-1}(m_n - d_n) \to \xi \in \mathbb{R}^{r}$ and let $U^{(n)}$ be a random vector with distribution $\mathcal{L}(V^{(n)} \,\mid\, M^{(n)} = m_n)$. Suppose that $\xi$ is an interior point of the support of $M$ and that there exists a version of $m \mapsto \mathcal{L}(V \,\mid\, M = m)$ continuous at $m = \xi$ as a function of $m \in \mathbb{R}^{r}$ into $\mathcal{P}(\mathbb{R}^{q})$, the set of probability measures of $\mathbb{R}^{q}$. Then,
  \begin{align}
    a_{n}^{-1} \left( U^{(n)} - b_n \right) \xrightarrow{\mathcal{D}} \mathcal{L}(V \,\mid\, M = m).
  \end{align}
\end{thm}

\begin{cor}[Corollary 2.5 of \cite{Janson:2007dx}]\label{cor:linear_op}
  We can replace the assumption above that $V^{(n)}$ is stochastically monotone with respect to $M^{(n)}$ by the assumption that $H V^{(n)}$ is stochastically monotone with respect to $M^{(n)}$ for some invertible linear operator $H$ on $\mathbb{R}^{d}$.
\end{cor}
\begin{proof}
  Apply the theorem to $(H V^{(n)}, M^{(n)})$ with $V$ and $b_n$ replaced by $HX$ and $H b_n$, respectively. The result follows by applying $H^{-1}$.
\end{proof}
% \hl{We are almost done with the proof.}
The number of unbalanced triangles is not stochastically monotone with respect to the number of negative ties in each stratum, so we cannot apply this theorem directly to $V^{(n)}_{p}$. It is not hard to see, however, that the counts of triangles having at least $\alpha=1,2,3$ negative ties satisfies stochastic monotonicity. 
Let $T_\alpha^{(n)}$ denote the number of triangles in $G_p^{(n)}$ with $\alpha$ negative ties.
Then, we have the following result:
\begin{lem}\label{lem:stoch_mono}
The vector $H T = (T_{3}, T_{3} + T_{2}, T_{3} + T_{2} + T_{1})$ is stochastically increasing with respect to $M$, where $T\coloneqq(T_{1}, T_{2}, T_{3})$, $M\coloneqq(M_{0}, \ldots, M_{L})$ and the matrix $H$, given by $Hx=(x_3,x_3+x_2,x_3+x_2+x_1)$ for $x\in \mathbb{R}^{3}$, is invertible.
\end{lem}
The proof is deferred to \Cref{sec:appendix_lemmas}.
% Consider the corresponding random variables $T^{(n)}$ and $T^{(n)}_\alpha$ with respect to $G^{(n)}_p$.
Since $H$ is an invertible linear operator, and $V^{(n)}_{p} = T_{1}^{(n)} + T_{3}^{(n)}$, \Cref{cor:linear_op} and \Cref{lem:stoch_mono} together shows that it is sufficient to prove a CLT for $(T^{(n)}, M^{(n)})$.
% it follows from \Cref{lem:stoch_mono}
% and \Cref{cor:linear_op}
% that $T^{(n)}$ is also stochastically decreasing with respect to $M^{(n)}$ (see Corollary 2.5 of \citet{Janson:2007dx}).
% Since $V^{(n)}_{p} = T_{1}^{(n)} + T_{3}^{(n)}$, it now suffices to prove a CLT for $(T^{(n)}, M^{(n)})$.
This requires a few mild assumptions.

% \begin{ass}\label{ass:increasing_levels}
%   We require the following terms to be increasing: the total number of triangles, and the number of negative edges in each embeddedness level, i.e.
%   \begin{align}
%     \abs{\triangle} &\to \infty, \qquad
%     m_l \to \infty,
%   \end{align}
%   for $l = 0, 1, \ldots L,$ as $n \to \infty$.
% \end{ass}
% \begin{rmk}
%   These assumptions are necessary conditions for the variance of our terms to diverge. After all, without triangles or negative ties, there is no balance.
%   % This assumption is a necessary condition for the variance of the $M_l^{(n)}$ terms to diverge, and is very mild, and is satisfied in almost all random graph models.
% \end{rmk}

\begin{ass}\label{ass:max_emb}
  The embeddedness level of negative ties in $\left\{ G^{(n)} \right\}_{n = 1}^{\infty}$ is bounded from above by some $L_{-} < \infty$.
\end{ass}

% \todo{check the maximum $L$ for the village}
Our first assumption is predominantly a technical one, as Nerman's Theorem does not apply when $L^{(n)}$, the dimension of $M^{(n)}$, is unbounded. Note that, under the current definition of $L^{(n)}$, which we recall is the largest embeddedness value in the graph $G^{(n)}$, we would require an upper bound on the embeddedness level of all ties (not just negative ties). But in fact it suffices to define $M^{(n)}$ up to the largest embeddedness level for negative ties (say $L_{-}^{(n)}$), as the permutations above $L_{-}^{(n)}$ (with no negative ties) would be degenerate.

% \footnote{Though it should be possible to extend Nerman's Theorem to infinite-dimensional distributions.}.
% On the other hand, it implies that the number of triangles is at most of order $O(n)$, because, according to the definition of embeddedness,
% \begin{align}
% 	\sum_{(i,j,k) \in E^3} \I{ (i,j,k) \in \triangle} = 2 \sum_{i \in E} \varepsilon_{i} = 2 \sum_{l=0}^L n_ll \leq 2Ln. \label{eqn:orderTriangles}
% \end{align}
% Accompanying Assumption 1, we make the following cosmetic adjustment to our permutation procedure. Instead of performing permutations on every embeddedness level present in the graph, it suffices to only apply permutations to embeddedness levels of at most $L^{-}$, where $L^{-}$ is defined as the maximum embeddedness level across all negative ties.
% Currently we are running permutations in every level of embeddedness present in the graph, even if there are no negative ties in that level.
% Our modification is to only apply permutations to embeddedness levels of at most $L$.
% This permutation is equivalent to our original one, since there are no negative ties in levels above $L^{-}$, and so such permutations are necessarily degenerate.
% Accompanying \Cref{ass:max_emb} we make the following minor adjustment to our permutation procedure. Instead of performing permutations on every level of embeddedness level present in the graph%
% \footnote{Many levels might have no negative ties, which renders the permutation step for that level moot.}%
% , we shall only apply permutations to embeddedness levels of at most $L$.
% Currently we are running permutations in every level of embeddedness present in the graph, even if there are no negative ties in that level.
% Our modification is to only apply permutations to embeddedness levels of at most $L$.
% As there are no negative ties in levels above $L$, such permutations are degenerate.
% The advantage afforded by this modification is that it makes no restrictions on the maximum embeddedness level of positive ties.
% Notationally, this means that $E$ no longer reflects all edges in $G$, but only those edges having embeddedness $\leq L$.

Moreover, in practice, the embeddedness level does not grow with the size of the graph.
For instance, across the 32 village networks in our dataset (with the number of edges ($n$) ranging from 54 to 1109), the largest embeddedness for negative ties was 5, while the largest embeddedness for positive ties was 13.
In fact, the largest graph (with 1109 edges) had a maximum embeddedness for negative ties of only 2.

% The advantage afforded by this adjustment is that we now no longer need to make any restrictions on edges of embeddedness level larger than $L$.

% Additionally, the upper bound is only on the largest embeddedness level that \emph{negative ties} are allowed to have%
% Additionally, the assumption is only on the largest embeddedness level that a negative tie is allowed to have,
% , making no restrictions on the largest embeddedness level of positive ties.
% -- it makes no restrictions on the largest embeddedness level on the graph.

% As a result, we will make the following slight adjustment to the permutation procedure:we shall restrict our stratified permutations to those with an embeddedness level at most $L$. As there will never be negative ties having embeddedness level more than $L$, permuting those levels are meaningless.
% The advantage afforded by this adjustment is that we now no longer need to make any restrictions on edges of embeddedness level larger than $L$.
% Notationally, this means that $E$ no longer reflects all edges in $G$, but only those edges having embeddedness $\leq L$.

% \begin{ass}\label{ass:lower_bound_p_l}
%   There exists a lower bound on the sequences $\left\{ p_l^{(n)} \right\}_{n = 1}^{\infty}$ for $l = 0, \ldots, L$. In other words, $m_l$ is at the same order as $n_l$. \textcolor{red}{RA You still change this, right? Or at least give a remark that some $p_l$ being zero in the limit is fine, because then we can just ignore the corresponding levels of embeddedness.}
%   % The $p_{l}^{(n)}$ terms satisfy the following lower bound:
%   % \begin{align}
%   %   p_{l}^{(n)} \gtrsim \frac{1}{n^{1/5}}, \quad l = 0, \ldots, L.
%   % \end{align}
%   % In other words, the order of $m_l$ is at most $\frac{1}{n^{1/5}}$ off the order of $n_l$.
% \end{ass}
% \begin{rmk}
%   In light of the adjustment outlined above, this is a mild assumption, as it simply requires the non-degenerate embeddedness levels to be bounded from below.
%   % This is a reasonable assumption as the case of the $p_l$'s converging to zero results in a degenerate scenario where $T_1^{(n)}$ dominates $T_{3}^{(n)}$.
% \end{rmk}

\begin{ass}\label{ass:emb2}
  We require $\sup_{i \in E} \varepsilon_i^2 = o(n).$
\end{ass}

\begin{ass}\label{ass:all_embed_limit}
  For $l_{1}, l_{2}, l_{3} = 0, \ldots, L_{-}$ define $E_{l_1,l_2,l_3} \coloneqq E_{l_1}\times E_{l_2}\times E_{l_3}$.
  % , $E_{l_2,l_3}=E_{l_2}\times E_{l_3}$.
  We assume that all partial sums
  \begin{align}
    \frac{1}{n} \sum_{(i,j,k) \in E_{l_1,l_2,l_3}} \triangle_{ijk},
    \qquad
    \frac{1}{n} \sum_{i \in E_{l_1}}
    % \left( \sum_{\substack{ j \in E_{l_2},\, k \in E_{l_3} }} \triangle_{ijk} \right)^2,
    \left(\sum_{(j,k) \in E_{l_2,l_3}}
    \triangle_{ijk}\right)
    \left(\sum_{(j',k') \in E_{l_4,l_5}}
    \triangle_{ij'k'}\right),
  \end{align}
  converge to a limit as $n \to \infty$, where $\triangle_{ijk} \coloneqq \I{(i,j,k) \in \triangle}$.
  Separately, we require $p_{l} = \dfrac{m_l}{n_l}$ to also converge to a limit as $n \to \infty$.
  % Note that we do not restrict these limits to be non-zero.
\end{ass}
This assumption is needed to ensure that the limiting covariance terms exist.
  % In most random graph models, the support of the graph is the main thing being modelled.
  % In our case, we have a fixed support. As a result, 
  We require such a condition because our statistic is intimately related to the structure of the sequence $\left\{ G^{(n)} \right\}_{n=1}^{\infty}$, which is fixed. This contrasts with other random graph models where the support of the graph is the main modeling task.
  % The reason for the existence of such a condition is that the important terms are functions of the underlying structure of $G$, which is fixed.
  % This is very different from the 
  % As a result, these conditions are needed to ensure an actual limit exists.
  A simple consequence of \Cref{ass:all_embed_limit} is that $\dfrac{n_l}{n}$ also converges, as
\begin{align}
  \frac{1}{2l}
  \sum_{l_2, l_3 = 0}^{L_{-}} \frac{1}{n} \sum_{(i,j,k) \in E_{l,l_2,l_3}} \triangle_{ijk}
  &= \frac{2}{2nl}  \sum_{i \in E_{l}} \varepsilon_i =  \frac{1}{nl} n_l l = \frac{n_l}{n} \label{eqn:n_l}
\end{align}
shows that $\dfrac{n_l}{n}$ is a finite, linear combination of terms that converge.
% According to \cref{eqn:orderTriangles} the means of $T^{(n)}_\alpha$ are of order $O(n)$.
% The proof of \Cref{prop:clt_radamacher} shows that the variances are of order $O(n)$.
% Consider therefore the random variables $\widetilde{T}^{(n)} \coloneqq \frac{1}{\sqrt{n}}{\left(T^{(n)} - \E{T^{(n)}} \right)}$, $\widetilde{M}^{(n)} \coloneqq \frac{1}{\sqrt{n}}{\left(M^{(n)} - \E{M^{(n)}} \right)}$. 
Consider therefore the normalized random variables $\widetilde{T}^{(n)} \coloneqq \frac{1}{\sqrt{n}}{\left(T^{(n)} - \E{T^{(n)}} \right)}$, $\widetilde{M}^{(n)} \coloneqq \frac{1}{\sqrt{n}}{\left(M^{(n)} - \E{M^{(n)}} \right)}$, where we recall that the variables $T^{(n)} = (T^{(n)}_{1}, T^{(n)}_{2}, T^{(n)}_{3})$ relate to the independent graph model $G_{p}^{(n)}$.

\begin{prop}\label{prop:clt_radamacher}
 Under \Cref{ass:max_emb,ass:emb2,ass:all_embed_limit}, we have for $n \to \infty$,
  \begin{align}
    \left( \widetilde{T}^{(n)}, \widetilde{M}^{(n)} \right) \xrightarrow{\mathcal{D}} \left( \widetilde{T}, \widetilde{M} \right)
    \sim \mathcal{N}(0, \Sigma),
  \end{align}
  where $\Sigma$ is given in \cref{eqn:sigma3} of \Cref{sec:appendix_proof}.
\end{prop}

\begin{rmk}
  As $\Sigma$ is an asymptotic variance, in practice, it is enough to approximate $\Sigma$ by the covariance matrix $\Sigma^{(n)}$ of $(\widetilde{T}^{(n)}, \widetilde{M}^{(n)})$, as given in \cref{eqn:sigma2} of \Cref{sec:appendix_proof}, using \cref{eqn:cov_t1,eqn:cov_t2,eqn:cov_t3,eqn:cov_t_m,eqn:cov_m}.
\end{rmk}


% essentially, i need the variance of the M's to not become degenerate. the variance is given by 1/n n_l p_l (1 - p_l) = m_l (1 - p_l), I need m_l / n > 0 \iff m_l / n_l > n_l / n \iff p_l > n_l / n
% if m_l / n is constant, then necessarily we have m_l / n_l and n_l / n being constants, duh, since there's an ordering.
% so actually we require both p_l and n_l / n to be constant.

The proof is deferred to \Cref{sec:appendix_proof}.
We are now ready to state and prove our main theorem.
\begin{thm}\label{thm:main}
  Grant \Cref{ass:max_emb,ass:emb2,ass:all_embed_limit}.
  % Under the mild conditions laid out in \Cref{ass:increasing_levels} and \Cref{ass:sup_bound}, the normalized count of unbalanced triangles is asymptotically normal, under $H_{0}^{\pi}$.
  Under the new null hypothesis, $H_{0}^{\pi}$,
  we have for $n \to \infty$ that the normalized count of unbalanced triangles has a limiting normal distribution:
  % as the number of edges $n \to \infty$,
  \begin{align}
    % \frac{1}{\sqrt{n}}
    n^{-1/2}\left( U^{(n)}_{\pi} - \E{ V^{(n)}_p } \right) \xrightarrow{\mathcal{D}} \mathcal{N}(0, \sigma^2_{u}),
    % \widetilde{U}^{(n)} \xrightarrow{\mathcal{D}} \widetilde{U} \sim \mathcal{N}(\mathbf{0}, \Sigma^{u}),
  \end{align}
  % where $\widetilde{U}^{(n)} = n^{-1}(U^{(n)} - \E{ V^{(n)} })$,
  with $\sigma^2_{u} = \Sigma^{s}_{1,1} + \Sigma^{s}_{3,3} + 2 \Sigma^{s}_{1,3}$ and $\Sigma^{s} = \Sigma_{\widetilde{T},\widetilde{T}} - \Sigma_{\widetilde{T},\widetilde{M}} \Sigma_{\widetilde{M},\widetilde{M}}^{-1} \Sigma_{\widetilde{T},\widetilde{M}}^{\top}$, where $\Sigma_{\widetilde{T},\widetilde{T}}$, $\Sigma_{\widetilde{M},\widetilde{M}}$ and $\Sigma_{\widetilde{T},\widetilde{M}}$ are the covariance matrices of $\widetilde{T}, \widetilde{M}$ from \Cref{prop:clt_radamacher}.
  % \todo{make it explicit, the term can be calculated from the graph sequence, so that one can actually implement this, when calculating the distribution}
  % with the form of $\Sigma^{u}, a_n, b_n$ to be provided later in this section.
\end{thm}

\begin{proof}
  \Cref{prop:clt_radamacher} gives us joint asymptotic normality of $(\widetilde{T}^{(n)}, \widetilde{M}^{(n)})$. 
  % Having the CLT of the Radamacher version (\Cref{prop:clt_radamacher}) and
  By stochastic monotonicity of $(T^{(n)}, M^{(n)})$ (\Cref{lem:stoch_mono}), we can apply Corollary 2.5 of \citet{Janson:2007dx} (a variation of Nerman's Theorem) to get
  \begin{align}
    \widetilde{S}^{(n)} \coloneqq \mathcal{L}\left( \widetilde{T}^{(n)} \,\mid\, \widetilde{M}^{(n)} = 0 \right) \xrightarrow{\mathcal{D}} \mathcal{L}\left( \widetilde{T} \,\mid\, \widetilde{M} = 0 \right).
  \end{align}
  Since $(\widetilde{T}, \widetilde{M})$ has a joint normal distribution, it is well known that the conditional distribution is also normally distributed. In other words, $\widetilde{S}^{(n)} \xrightarrow{\mathcal{D}} \widetilde{S} \sim N(0, \Sigma^{s})$ and, in particular,
  \begin{align}
    % \frac{1}{\sqrt{n}}
    n^{-1/2}
    \left( U^{(n)}_{\pi} - \E{V^{(n)}_{p}} \right) = \widetilde{S}^{(n)}_{1} + \widetilde{S}^{(n)}_{3} \xrightarrow{\mathcal{D}} \mathcal{N}(0, \sigma^2_{u}).
  \end{align}
\end{proof}

% \thought{the asymptotic means of U and V coincide, }
% \todo{say more here thanks}
% \begin{rmk}
%   The asymptotic means of $U^{(n)}$ and $V^{(n)}$ coincide.
% \end{rmk}

\begin{rmk}
  Note that $\widetilde{M}_l^{(n)}$ is degenerate if $\frac{m_l}{n} \to 0$.
  % This poses a potential problem as we are conditioning on the $\widetilde{M}_l^{(n)}$ random variables.
  % In order for $\widetilde{T}^{(n)}$ to be non-degenerate, 
  % Note that $\widetilde{T}^{(n)}$ is degenerate when $\abs{\triangle} = o(n)$, which occurs when $\frac{n_l}{n}$ converges to 0 for all $l > 0$.
  % which happens if $\liminf_{n\rightarrow \infty} p^{(n)}_0 >0$ while all other $p_l$ converge to $0$. Otherwise, we always have $\abs{\triangle}\asymp n$. On the other hand, $p_l\rightarrow 0$ means that $\widetilde{M}_{l}^{(n)}$ becomes degenerate and therefore also $\widetilde{M}^{(n)}$.
  %in which case it makes sense  to assume that $\abs{\triangle} \asymp n$. 
  %However, even under this assumption, the individual $M_l$'s terms can still become degenerate, when $m_l = o(n)$. 
  To ensure that we don't invert a degenerate covariance matrix, we can simply remove the degenerate $\widetilde{M}_l^{(n)}$ from $\widetilde{M}^{(n)}$. The result still holds, as stochastic monotonicity is maintained with the smaller $\widetilde{M}^{(n)}$.  
\end{rmk}

  From the form of the limiting distribution, it is clear that the asymptotic means of $U^{(n)}_{\pi}$ and $V^{(n)}_{p}$ coincide (though the variances differ).
  % \textcolor{red}{RA proof for this? It's obvious for us, but not clear to the reader. Also, here and in the proof probably better write $U_{pi}^{(n)}$}
  % This raises the question of why we even bother using the permutation model
  This suggests that one could save a lot of trouble by adopting the independent model $G_{p}$ instead of using the permutation model $G_{\pi}$, with little difference in results besides some \hl{inevitable increase} in variance.
  This is indeed true when the size of the graph is very large, but for the rest, like the graphs we collected in our dataset, the discrepancy between the two models is nontrivial.
  In particular, due to the small size of our graphs, and the small number of negative ties observed, empirically we find that the graphs generated under the independent model will often have no negative ties, rendering the task of measuring balance moot.


As a byproduct, we also obtain asymptotic normality for $U^{(n)}_{\tau}$ in the old model.
\begin{cor}\label{cor:an_uniform}
  Asymptotic normality of $U^{(n)}_{\tau}$, the statistic under \Cref{modl:old}, follows from \Cref{thm:main}, by replacing the vector $M^{(n)}$ by the sum $\sum_{l = 0}^{L_{-}} M_{l}^{(n)}$, and letting $p_{\varepsilon_i} = \frac{m}{n}$ for all $i \in E$.
  % Many of the assumptions will also be simplified, as the $p_{\varepsilon_i}$'s are now identical.
\end{cor}

\begin{rmk}
  The proof of \Cref{lem:cond_dist} requires only that the probabilities for an embeddedness level are identical (i.e. $p_i = p_j \text{ if } \varepsilon_i = \varepsilon_j$). In particular, this means that one could also choose $p_{\varepsilon_i} = \frac{m}{n}$ for all $i \in E$. By doing so, one could start with the same independent graph random variable, and then we can recover both permutation random variables, depending on if we were to condition on each embeddedness level separately ($M = \left\{ m_i \right\}_{i=1}^{L_{-}}$) or on the total number of negative ties ($M = \sum_{i = 1}^{L_{-}} m_i$).

  However, if we were to use the random graph with uniform probability $\frac{m}{n}$ of being negative, then the event that we condition on, $\left\{ M^{(n)} = \bm{m}^{(n)} \right\}$, is not at the mean of the distribution (recall that we are forced to condition on the empirical counts of the embeddedness levels). Thus the statement of our theorem becomes degenerate as, in the limit, $\P{ M = \bm{m}} = 0$.
\end{rmk}

\subsection{Comparison of the two Models}
\label{sub:comparing_both}

% how to sell this section?
% result: we show type-I error for an increasingly general sequence of models
% issue: we need all these approximations, because it's very difficult

% The goal of this section is to provide some theoretical justification for our test.
% % The goal here is to derive some theoretical results showing the superiority of our test to the old test.
% We shall do so by considering the Type-I error of the two tests under reasonable definitions of balance-free graphs.
% We will start with the null distribution that our test uses, but from that result we will then extend it to more general null distributions. 
% Getting exact details would be nigh impossible, as the distribution of the statistic does not have a closed form.
% Thus, we shall use the normal approximations to the null distributions as a proxy. 

We have argued in \Cref{sec:method} that a graph can be considered balance-free, if the sign of an edge is independent of its position in the graph, relative to its embeddedness. Among other issues, ignoring embeddedness means treating all edge labels as exchangeable which is not true for social networks. We concluded that reasonably balance-free graphs can be generated with respect to the restricted random permutation $\pi$. Building on this idea, in this section we will construct a hierarchy of generative models producing balance-free graphs and show, if these graphs are assumed as null models, that the old test with respect to the critical values $c_{\alpha,\tau}^{(n)}$ derived from \Cref{modl:old} has Type-I error converging to 1 as $n \to \infty$, while our test with critical values $c_{\alpha,\pi}^{(n)}$ from \Cref{modl:new}  has Type-I error matching the specified $\alpha$. This proves formally that the new test is more conservative than the old one. \Cref{sec:simulations} will show, on the other hand, that the new test still detects balance, if it exists. 

Arguing by the normal approximations in \Cref{thm:main} and \Cref{cor:an_uniform}, comparing the critical values essentially reduces to comparing the means and variances of Gaussians. This yields the following result.
\begin{prop}\label{lem:old_test_fails}
Grant \Cref{ass:max_emb,ass:emb2,ass:all_embed_limit} and assume that there exists a constant $c>0$ such that for large $n$
\begin{align}
    (1-p)^2 \frac{\sum_{i \in E} \varepsilon_i}{n} - \frac{ \sum_{i \in E^{-}} \varepsilon_i }{m} > cm^{1/2}\log{m}, \label{eqn:difference_means}
\end{align} 
where $E^{-}\subset E$ is the set of negative ties in $G^{(n)}$. 
Then $\P{U^{(n)}_{\pi}\leq c_{\alpha,\pi}^{(n)}}\rightarrow \alpha$, while $\P{U^{(n)}_{\pi}\leq c_{\alpha,\tau}^{(n)}} \rightarrow 1$ as $n \to \infty$, i.e. the Type-I error of the original test applied to graphs generated by $G^{(n)}_{\pi}$ converges to 1.
\end{prop}

The proof is deferred to \Cref{sec:appendix_lemmas}. Observe that \cref{eqn:difference_means} requires the difference in the average embeddedness values of all ties versus just negative ties to have enough separation. These two terms essentially reflect the means of the two distributions.

% Now, let us generalize the model. Instead of using the stratified permutation, the same results hold if we are under the Rademacher model $G_{p}^{(n)}$. To see why, recall that the permutation model can be obtained by conditioning of the Rademacher model (\Cref{lem:cond_dist}). From \Cref{lem:old_test_fails} it follows that the Type-I error for the old test under $G^{(n)}_{\pi}$ converges to 1. Since the Type-I error for $G^{(n)}_{p}$ is a weighted average of these terms, it must also converge to 1 as $n \to \infty$.

Now, let us generalize the model. Instead of using the stratified permutation, the same results hold if we replace $G_{\pi}^{(n)}$ with the Rademacher model $G_p^{(n)}$.
% To see why, recall that the permutation model can be obtained by conditioning on the Rademacher model (\Cref{lem:cond_dist}).
% A little care must be taken here.
Recall that the new test derived from \Cref{modl:new} (and the respective critical value) depends only on $\bm{m}^{(n)}$ (provided the support of the graph is fixed). Now, graphs generated from $G_{\pi}^{(n)}$ all have the same value of $\bm{m}^{(n)}$ so they all share the same critical value. However, when we generalize to $G_{p}^{(n)}$, then the critical value will be a function of the $\bm{m}^{(n)}$. Let us denote the critical value by $c_{\alpha,\pi}(\bm{m}^{(n)})$. Then, 
% Consider the random graph sequence $G_{p}^{(n)}$. Then, for $c > 0$,
\begin{align}
  % c_{\alpha, \pi}(\bm{m}^{(n)})
  \P{ V_{p}^{(n)} \leq c_{\alpha,\pi}(\bm{m}^{(n)})}
  &= \sum_{\bm{m}^{(n)}} \P{ V_{p}^{(n)} \leq c_{\alpha,\pi}(\bm{m}^{(n)}) \,\mid\, M^{(n)} = \bm{m}^{(n)}} \P{ M^{(n)} = \bm{m}^{(n)} }
  \\&= \sum_{\bm{m}^{(n)}} \P{ U_{\pi}^{(n)} \leq c_{\alpha,\pi}(\bm{m}^{(n)})} \P{ M^{(n)} = \bm{m}^{(n)} }  \label{eqn:crit_error}
  \\&= \sum_{\bm{m}^{(n)}} \alpha \cdot \P{ M^{(n)} = \bm{m}^{(n)} }.
  % \\&= \sum_{\bm{m}^{(n)}} \alpha \P{ \bm{M}^{(n)} = \bm{m}^{(n)} } = \alpha
\end{align}
% Substituting the critical value for the new test, \cref{eqn:crit_error} reduces to
% \begin{align}
%   \P{ V_{p}^{(n)} \leq c_{\alpha, \pi}(\bm{m}^{(n)}) }
%   &= \sum_{\bm{m}^{(n)}} \alpha \P{ M^{(n)} = \bm{m}^{(n)} } = \alpha.
% \end{align}
On the other hand, considering the critical value for the old test, \cref{eqn:crit_error} would be
\begin{align}
  \P{ V_{p}^{(n)} \leq c_{\alpha, \tau}(\bm{m}^{(n)}) }
  &= \sum_{\bm{m}^{(n)}} \P{ U_{\pi}^{(n)} \leq c_{\alpha, \tau}(\bm{m}^{(n)})} \P{ M^{(n)} = \bm{m}^{(n)} }.
\end{align}
By \Cref{lem:old_test_fails}, we have that for each term, $\P{ U_{\pi}^{(n)} \leq c_{\alpha, \tau}(\bm{m}^{(n)})} \to 1$ as $n \to \infty$. Thus, since $\sum_{\bm{m}^{(n)}} \P{ M^{(n)} = \bm{m}^{(n)} } = 1$, we have that $ \P{ V_{p}^{(n)} \leq c_{\alpha, \tau}(\bm{m}^{(n)}) } \to 1$ as $n \to \infty$ as required.

% The above calculation follows from the simple observation that, for a fixed underlying graph $G$, the critical value derived from \Cref{modl:old} (the uniform model) is only a function of the $m = \sum_{i} m_i$, while the critical value derived from \Cref{modl:new} is a function of the individual $m_i$'s.

% The same result also holds for $H_{0}^{p}: \mathbf{G} \sim G_{p}$. To see why, according to Lemma  \Cref{lem:cond_dist}), we can apply the above result for each fixed $\left\{ m_l \right\}_{l=0}^{L}$ to get that the Type-I error converges to 1, and so this holds uniformly.

% Moving from $H_0^{\pi}$ to $H_0^{p}$ removes the restriction of the number of negative ties. However, we are still forced to have the same support for each graph. The 
% Finally, we can generalize the balance-free graph model $G_p$ even further by expanding the set of possible locations of negative ties to outside the support of $G$. In other words, every $2^{|V|}$ possible edges has probability $p_{\varepsilon_i}$ of being negative.
% For those locations without an edge present, one can define a \emph{pseudo}-embeddedness value, by the number of triangles that would be added if there was an edge in that location.
% One can weaken the assumptions of the above model even further by expanding the set of possible locations of negative ties to outside the support of $G$, 
% One can further weaken the assumptions of the above model, and expand the set of possible locations of negative ties to empty ties, making sure to stay faithful to the embeddedness levels.
% The only caveat is that the support of the graph now varies between samples, but since the variability is minimal, the results should still hold.

Finally, we can generalize the balance-free graph model $G_p^{(n)}$ even further to consider general graphs (that is, no longer confined to a fixed support). This can be achieved by simply adding an additional step to the generative model: first randomly draw a unsigned graph $G$ (the support) from some distribution over all possible graphs on $N$ vertices, then draw from $G_p^{(n)}$. A similar argument to the one above gives the result.


% \begin{prop}
%   Consider the following generating process for a graph without balance: fix a positive subgraph $G$, then generate the negative subgraph as an \ER graph (we shall revisit this in \Cref{sec:simulations}).
%   If there is a collision, the negative tie takes precendent.
%   Then, the same result holds for this model.
% \end{prop}
% \begin{proof}
% % [Sketch of proof]
%   % Aside from the issue of what happens when the negative and positive ties collide,
%   This is very close to $H_{0}^{p}: G \sim G_{p}$, except that now the set of possible places that a negative tie can go are the empty positions.
%   The one caveat is that the $G$ now varies between samples.
% \end{proof}

% We shall work our way up to a reasonable model, but let us start with a somewhat contrived example. Suppose the true null model for graphs without the mechanism of balance is given as follows: fix a graph $G$ and sequence $\left\{ m_l \right\}_{l = 0}^{L}$. Then, the generative process is simply to randomly assign negative weight to $m_l$ edges having embeddedness $l$. This is basically the null hypothesis that we use, hence why it is a \emph{contrived} example.

% Now, this setting is nice because the null model that our method (and consequently also the old method) forms matches the true null model, since our methods only depend on $G$ and $\left\{ m_l \right\}_{l = 0}^{L}$.
% Let us analyze the Type-I error. In our case, the distribution of the statistic is exactly the same as the distribution of the null, so the Type-I error matches our significance level. This is not the case for the old method.

% Now consider the following relaxation. Instead of fixing the $m_l$'s, we instead let $M_l \sim \operatorname{Bin}\left( n_l, p_l \right)$ (this now corresponds to the Radamacher model we have). However, we already know that the permutation distribution is simply a conditional distribution on the event $\left\{ M_l = m_l \right\}_{l = 0}^{L}$. Thus, for each fixed $\left\{ m_l \right\}$ we have that the Type-I error of the old method is converging to 1, this then holds under this model too.
% \todo{do i have things reversed?}

% Finally, to see why this model is not so unreasonable, consider a different generating process for graphs without balance: we fix a positive subgraph $G$, and then generate the negative subgraph as an \ER graph. We shall revisit this when we detail our simulations (\Cref{sec:simulations}).
% But, aside from the issue of what happens when the negative and positive ties collide, this is very close the model as the one above\todo{these should have names}, except that now the set of possible places that a negative tie can go are the empty places with embeddedness $l$. The caveat is that the $G$ is now changed between samples of the generative model.

